ExpFinder: An Ensemble Expert Finding Model Integrating $N$-gram Vector Space Model and $\mu$CO-HITS

Finding an expert plays a crucial role in driving successful collaborations and speeding up high-quality research development and innovations. However, the rapid growth of scientific publications and digital expertise data makes identifying the right experts a challenging problem. Existing approaches for finding experts given a topic can be categorised into information retrieval techniques based on vector space models, document language models, and graph-based models. In this paper, we propose $\textit{ExpFinder}$, a new ensemble model for expert finding, that integrates a novel $N$-gram vector space model, denoted as $n$VSM, and a graph-based model, denoted as $\textit{$\mu$CO-HITS}$, that is a proposed variation of the CO-HITS algorithm. The key of $n$VSM is to exploit recent inverse document frequency weighting method for $N$-gram words and $\textit{ExpFinder}$ incorporates $n$VSM into $\textit{$\mu$CO-HITS}$ to achieve expert finding. We comprehensively evaluate $\textit{ExpFinder}$ on four different datasets from the academic domains in comparison with six different expert finding models. The evaluation results show that $\textit{ExpFinder}$ is a highly effective model for expert finding, substantially outperforming all the compared models in 19% to 160.2%.

==> Expertise Retrieval_TKDE/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we proposed \EF a novel ensemble model for expert finding. We presented the design of \EF and conducted comprehensive empirical experiments to evaluate and validate its effectiveness using 
four publicly accessible datasets (LExR~\cite{Vitor:2016}, Information Retrieval, Semantic Web and Computational Linguistics in DBLP dataset \citep{bordea2013benchmarking}) from the academic domains.  The novelty  of \EF is in its incorporation of a novel $N$-gram vector space model ($n$VSM) into \hits. The key to designing $n$VSM is to utilise the state-of-the-art IDF method~\citep{nidf:2017} for estimating the topic-sensitive weights of experts given a topic. 
Such estimated weights are further improved by incorporating them into \ecg using \hits. Our novelty of \hits is to design two variation schemes of CO-HITS~\cite{Hongbo:2009}, thus proposing a unified formula for successfully integrating $n$VSM with \hits. We showed comprehensive evaluation, comparing \EF with the six representative models, that is,  TF-IDF based vector space models (TFIDF), two document language models (DLM) \cite{Balog:2009, WISER:2019},  two graph-based models (GM)~\citep{Gollapalli:2013,Daniel:2015}, and topic-sensitive CO-HITS~\cite{Hongbo:2009}. We showed  \EF is a highly effective ensemble model for expert finding, outperforming TFIDF with 35.9\%, DLMs with 71.5\% - 160.2\%, GMs with 31\% - 129.1\%, and topic-sensitive CO-HITS with 19.0\%. 

%. Moreover, we showed how  we choose best parameters for \EF  using an  empirical  analysis on the four datasets. This would provide a potential benefit for researchers within the community to reuse \EF for expert finding in other domains. Further, we evaluated the impact of \hits within \EF over the $n$VSM and the CO-HITS algorithm~\cite{Hongbo:2009} for expert finding. Overall, our evaluation showed that \EF has high potential for expert finding, highly outperforming the compared DLM, VSM and GM methods for expert finding.



==> Expertise Retrieval_TKDE/design.tex <==

\section{Design of ExpFinder}\label{sec:design}
In this section, we present the details of the four steps for designing and developing \EF.

\subsection{Extract Topics} \label{sec: keyphrase}
% Domain-specific concepts are often described by noun phrases that represent the key information within a given corpus $\mc{D}$~\cite{Kang:2014}. 
% A noun phrase means a single-word noun or a group of words that function together as a noun. A kephrase is  one of  the $N$-top extracted noun phrases, where $N$ is a user-specified a parameter.
%However, we note that all noun phrases cannot be useful for accurately representing given text documents. A reason is that such phrases may contain noise terms or the terms that are too general and common~\cite{Kang:2014}. 
As presented in Section~\ref{sec:overview}. we assume that a topic is represented as a {noun phrase}. 
% Thus, keyphrase extraction is the fundamental for expertise retrieval in \EF. 
We perform the following steps to extract noun phrases from $\mc{D}$. First, for each document $d \in \mc{D}$, we split $d$ into its sentences keeping their sequential indices.
% as some keyphrase tools (e.g. YAKE!~\cite{YAKE:2020}) assume that the earlier phrases appeared are more important than the later phrases appeared in a document (i.e. YAKE! is using sentence indices). 
Second, for each sentence, we analyse POS tags of the words in the sentence and remove stopwords. POS tagging is the process for assigning a part of speech to each word in a sentence. Then, each word remained is converted into its lemmatised form. Lemmatisation is the process of grouping together the inflected forms of a word, thus they can be considered to be a single item (e.g. `patients' is lemmatised to `patient'). Third, in the sentence, we use the following linguistic pattern based on POS tags to extract noun phrases: 
\begin{equation}\label{eq:keyphrase}
{\rm (JJ)^*|(VBN)^*|(VBG)^*(N)^+},     
\end{equation}
where `${\rm JJ}$' means adjective, `${\rm VBN}$' past participle, `${\rm VBG}$' gerund, and `${\rm N}$' nouns. Using this pattern, we can extract a noun phrase starting with (1) one or more nouns; (2) one or more adjectives followed by one or more nouns (e.g. `medical system'); (3) one or more past participle followed by one or more nouns (e.g. `embedded system'); and (4) one or more gerund followed by one or more nouns (e.g. `learning system'). The symbol `*' denotes zero or more occurrences, `+' denotes one or more occurrences.

% Also, we remove a phrase surrounded by parentheses (i.e. `\{\}',`()',`[]'), if the phrase is a single-lECGth word, assuming that such word often represents an alternative form (or abbreviation) of the proceeding phrase.  For example, in a given sentence, `Natural Language Processing (NLP)' is replaced with `Natural Language Process ()' as `NLP' is the abbreviation of the proceeding phrase, `Natural Language Process'. Note that we keep the parentheses (i.e. `()') as a separator that splits `Natural Language Processing ()' with the rest of that sentence.
% Another rule applied for preprocessing is that the we detect possessive nouns and remove their `'s' (and `'' for a plural noun ending with an `s') to uniquely identify its original noun form.
% Finally, we remove stopwords and digits from each sentence, and apply lemmatisation on each word based on its Part-Of-Speech (POS) tags. POS tagging is the process for assigning a part of speech to each word in a sentence.
% According to the notations in Section~\ref{sec:notation}, the extracted keyphrases are denoted as $\mc{T}$ and also called `expertise topics'.

Note that \EF does not rely on a particular method for noun phrase extraction, and thus can incorporate any noun phrase extraction methods.
% That means \EF is independent on a particular keyphrase extraction method, and thus \EF is designed to incorporate any keyphase extraction methods.

\subsection{Estimate the weights of experts and documents given topics}\label{sec:ntfidf}
We now present the process for creating a topic-expert matrix $\mb{TX}$ and a topic-document matrix $\mb{TD}$ from the extracted topics using $n$TFIDF in $n$VSM. These matrices will be used as the input to \hits.

\subsubsection{Topic-Expert Matrix Creation}\label{sec:XT}
% We present how to create a $\mb{TX} \in \mathbb{R}^{|\mc{T}|\times|\mc{X}|}$,  where each entry reflects the weight of an expert $x \in \mc{X}$ for  a given topic $t \in \mc{T}$.
To create a $\mb{TX}$, our fundamental is to utilise the definition of the DLM~\cite{Balog:2009,Wang:2015} for expert finding. Thus, we first briefly describe how this DLM can measure the topic-sensitive weight of an expert $x \in \mc{X}$ given a topic $t \in \mc{T}$, denoted as $p(x|t)$. Formally, it is given as~\citep{Balog:2009}:
% by incorporating the following components into a uniform formula: the weight of a document $d \in \mc{D}$: $p(d)$, the relevance of $d$ to $t$: $p(t|d)$, and the association between $d$ and $x$: $p(x|d)$.
% The weight of $x$ with respect to $t$ is represented as follows~\citep{Balog:07}:
\begin{equation}\label{eq:pw}
    p(x|t) = {p(x, t)}/{p(t)},
\end{equation}
where $p(x, t)$ is the joint probability of $x$ and $t$, and $p(t)$ is the probability of $t$. We can ignore $p(t)$ as this is a consistently constant over all experts $\mc{X}$. Thus, $p(x|t)$ is approximated by $p(x,t)$ that is reformulated  considering documents $\mc{D}_x$~\cite{Balog:2009}:
\begin{equation}\label{eq:pw_2}
    \begin{split}
    p(x, t) &= \sum_{d \in \mc{D}_{x}}p(x, d, t) = \sum_{d \in \mc{D}_{x}}p(d)p(x, t|d)  \\
    &= \sum_{d \in \mc{D}_{x}}p(d)p(t|d)p(x|d).
    \end{split}
\end{equation}

In Eq.~\ref{eq:pw_2}, we observe the following notations~\citep{Wang:2015}:
\begin{itemize}
    \item $p(d)$ is the prior probability of $d$ that can also be interpreted as the weight (or importance) of $d$.
    % One way to estimate $p(d)$ is to use the citation information of $d$ for the last some years~\citep{Rodrigo:2019} and/or an impact factor of the publisher~\citep{Hwang:2010}.
    % and a time decaying factor penalising old documents~\citep{Zhang:2017}.
    % using a simple formula: 
    % \begin{equation}\label{eq:age}
    %     p(d) = {\exp^{-|age| * \alpha}} * p(d),
    % \end{equation}
    % where $age$ is the longevity of $d$ by calculating the year difference between its published year to the most recent published year of publications in $\mc{D}$, and $\alpha$ is a sensitive parameter, where the larger it is, the sooner old publications become unimportant.

    \item $p(x|d)$ is the conditional probability of $x$ given $d$ (e.g. in a simply way, it can be estimated based on the order of $x$ in the co-author list in $d$~\cite{Wang:2015}). 
    % Recall that the weight is represented by $\mb{DX}_{i(d),i(x)}$, where $i(d)$ and $i(x)$ indicate the index of $d$ and $x$ in the matrix $\mb{DX}$, respectively (see Section~\ref{sec:notation}). 
    \item $p(t|d)$ is the conditional probability of $t$ given $d$. 
\end{itemize}


In the DLM~\citep{Balog:2009,Wang:2015},  it is assumed that a document $d$ is described as a collection of terms that appear in $d$. An importance of a term $w \in t$ within $d$ is determined by the proportion of its occurrences. DLMs provide a way of capturing this notion by representing a document as multinomial probability distribution over the vocabulary of terms. 
To estimate $p(t|d)$, let $\theta_d$ be the document model of $d$, and the probability of $t$ in $\theta_d$ is $p(t|\theta_d)$. This $p(t|\theta_d)$ indicates how likely we see $t$ if we sampled $t$ randomly from $d$. Thus, $p(t|d)$ is rewritten as $p(t|\theta_d)$ taking the product of $t$'s individual term probabilities as follows~\cite{Balog:2009,Wang:2015}:  
\begin{equation}\label{eq:topic_by_terms}
    p(t|\theta_d) = \prod_{w\in t} p(w|\theta_d),
\end{equation}
where $w$ is an individual term in $t$. However, a limitation of Eq.~\ref{eq:topic_by_terms} is that unseen terms in $d$ would get a zero probability. Thus, it is a common in DLMs to introduce a \textit{smoothing} factor to assign non-zero probability to the unseen terms.
% , thus improving the accuracy of word probability estimation in practice.
Typically, it can be done by reducing the probabilities of the terms seen in the corpus and assigning the additional probability mass to unseen terms. Formally, $p(w|\theta_d)$ is re-expressed as:
\begin{equation}\label{eq:document_model}
    p(w|\theta_d) = (1 - \lambda_\theta) p(w|d) + \lambda_\theta p(w|\mc{D})
\end{equation}
where $p(w|d)$ is estimated by the term frequency of $w$ in $d$ divided by $|d|$ (the number of terms in $d$), denoted as $tf(w,d)$, and $p(w|\mc{D})$ is the term frequency of $w$ in $\mc{D}$ normalised by $|\mc{D}|$, i.e., ${tf(w, |\mc{D}|)}$. The parameter $\lambda_\theta$ controls the influence of the two probabilities.

We now present our novelty for estimating $p(t|d)$ using $n$TFIDF. Since $n$TFIDF is an extension of TFIDF, we briefly describe how $p(t|d)$ can be estimated using TFIDF in VSM.
In a sense, $p(t|d)$ can also be interpreted using TFIDF~\citep{Roelleke:08}. 
Note that TFIDF is a measure based on the distance between two probability distributions, expressed as the cross-entropy: (1) a \textit{local distribution} of $w \in t$ in $d$, and (2) a \textit{global distribution} of $w$ in $\mc{D}$. 
TFIDF is a measure of perplexity between these two distributions. 
% If the distribution of query words in a document is unusual given the distribution of words in the collection, this is unlikely to happen by chance. In other words, if the global distribution of words is perplexed by the distribution of query words in a document, such document can be relevant. Furthermore, 
A higher perplexity score implies a higher relevance of $d$ to $w$. The cross-entropy between distributions $p_w$ and $q_w$ is as follows:

\begin{equation}\label{eq:entropy}
    -\sum_w p_w \log q_w= \sum_w p_w \log \frac{1}{q_w},    
\end{equation}
if we substitute $p_w$ with ${tf(w,d)}$ (TF) and $\frac{1}{q_i}$ with the inverted probability of encountering $d$ with a term $w$ (IDF), denoted as $\frac{|D|}{df(w)}$, where $df(w)$ is the document frequency of $w$, we obtain a TFIDF formula:

\begin{equation}\label{eq:entropy2}
    p(t|d) \approx \sum_{w\in t} {tf(w,d)} \log \frac{|D|}{df(w)}.
\end{equation}
Thus, as highlighted in~\cite{lu2013insight}, VSM and DLM are actually closely related. The TF component ${tf(w,d)}$ is exactly same as the probability of seeing a term $w$ in DLM.
The IDF component $\frac{|D|}{df(w)}$ is implicitly related to a smoothing method in DLM that uses the collection frequency (${tf(w, |\mc{D}|)}$: term frequency of $w$ in $\mc{D}$ normalised by $|\mc{D}|$.


% Typically, such methods can be split by two approaches: (1) \textit{local term weighting} and (2) \textit{global term weighting}. The first approach assigns a weight to a term $w$ within a document, often using $w$'s frequency in the document. The latter approach uses global information that can be observed within the entire document collection, often using document frequency or total term frequency over the collection. Term Frequency-Inverse Document Frequency (TFIDF) has become a standard term weighting method that combines the above two approaches into a uniform formula for bag-of-words representation of texts. 

% Formally, in the TFIDF method, the weight of a term (single-word) $w$ in a document $d \in \mc{D}$ can be computed as follows:
% \begin{equation} \label{eq:tfidf}
% {\rm TFIDF} (w, d) = {tf}(w, d) \cdot \log\frac{|\mc{D}|}{df(w)},
% \end{equation}
% where $tf(w, d)$ is the term frequency of $w$ in $d$, $df(w)$ is the document frequency of $w$ over the corpus $\mc{D}$. 

Based on the above observation, we now present our approach for estimating $p(t|d)$ using $n$TFIDF in $n$VSM.
Although some variant forms of TFIDF methods have been proposed, the majority of TFIDF methods use the same IDF function~\citep{nidf:2017}.
However, one drawback of IDF is that it cannot handle $N$-grams, contiguous sequence of $N$ terms (for $N$$>$1). The reason is that IDF tends to give a higher weight to a term that occurs in fewer documents. Note that typically, phrases occur in fewer documents when their collocations are less common. Thus, uncommon phrases  (e.g. noise phrases) are unintentionally assigned high weight, yielding the conflict with the definition of a good phrase that constitutes a succinct conceptual descriptor in text. To address it, \textit{$N$-gram IDF} for weighting phrases was recently proposed~\citep{nidf:2017}. $N$-gram IDF has shown the ability to accurately estimate weights of dominant phrases of any length, simply using the domain corpus.

The key in $n$VSM is the proposed formula $n$TFIDF that uses a combination of the frequency of a topic $t$ with $t$'s $N$-gram IDF. As that frequency, we use the average frequencies of the constituent terms in $t$. Formally, using $n$TFIDF, $p(t|d)$ is defined as:

\begin{equation}\label{eq:ntfidf}
\begin{split}
    p(t|d) \approx &~n{\rm TFIDF} (t, d) = ntf(t, d) \cdot nidf(t), {\rm ~where} \\
    &ntf(t, d) = \frac{\sum_{i=1}^{n}{tf ({w_i, d}})}{|t|}, \\
    &nidf(t) =  \log \frac{|\mc{D}|\cdot df(t)}{df(w_1 \land w_2 \land ... \land w_n)^2}
\end{split}
\end{equation}
where $w_1, \ldots, w_n$ are $n$-constituent terms in $t$, 
$tf ({w_i,d})$ is the term frequency of $w_i$ in $d$ normalised by $|d|$, 
$|t|$ is equal to $n$, and $nidf (t)$ is the $N$-gram IDF method for $t$ \citep{nidf:2017}.
% , and it has been proven to be very stable for any $N > 1$ and show its robustness for the use of determining dominant phrases. 
Eq.~\ref{eq:ntfidf} applies for all $|t| \geq 1$, where $nidf(t)$ is equal to the log-IDF, $\log \frac{|\mc{D}|}{df(t)}$, in Eq.~\ref{eq:entropy2},  when $|t|$=1.

% Avoid 0 in dem => +1

Finally, in $n$VSM, $p(x|t)$ in Eq.~\ref{eq:pw_2} is calculated using $p(t|d)$ in Eq.~\ref{eq:ntfidf} and is stored into the entry $\mb{TX}_{i(t), i(x)}$, where $i(t)$ and $i(x)$ indicate the row and column index of $t$ and $x$, respectively, in the $\mb{TX}$.

% The value of $p(t|d)$ is given as $\mb{DT}_{d,t}$ that is estimated using Equation~\ref{eq:ntfidf}. The value of $p(t|\mc{D})$ is estimated as the average value of the $t$-th column values $\vec{\mb{DT}}_{*,t}$ in the matrix $\mb{DT}$ (see the notations in Section~\ref{sec:notation}). That is, the average value indicates the average value of all nTFIDF values of the topic $t$ over all publications $\mc{D}$.


% However, in our approach, we presented how we have measured the weight of the topic $t$ (keyphrase) using Equation~\ref{eq:ntfidf} in Section~\ref{sec:ntfidf}. Thus, each topic can seen as a single term that concatenates multiple words composing the topic with space characters. Therefore, the above Equation can be simply rewritten as:
% \begin{equation}
%     p(t|\theta_d) =  p(w|\theta_d),
% \end{equation}
% where $w$ is equal to $t$.

\subsubsection{Topic-Document Matrix Creation}\label{sec:PT}
To create a topic-document matrix $\mb{TD}$, we need to calculate the topic-sensitive weight of a document $d$  given a topic $t$. Following the idea of the DLM~\cite{Balog:2009} again, we can estimate this weight by calculating the probability of $d$ being relevant to $t$: $p(d|t)$. Using the Bayes theorem, $p(d|t)$ can be calculated as:

\begin{equation}\label{eq:pw_d}
    p(d|t) = {p(t|d) p(d)}/{p(t)},
\end{equation}
where  $p(t)$ can be ignored as it is a consistently constant over all documents. Thus, $p(t|d)p(d)$ can be calculated by multiplying  $p(t|d)$ in Eq.~\ref{eq:ntfidf} and $p(d)$.
Finally, $p(d|t)$ is stored into the entry $\mb{TD}_{i(t), i(d)}$, where $i(t)$ and $i(d)$ indicate the row and column index of $t$ and $d$, respectively, in the $\mb{TD}$.

\subsection{Construct an ECG}
Although we have estimated the topic-sensitive weight of an expert $x$ for a given topic $t$ in $n$VSM, one potential limit may be that $p(x|t)$ in Eq.~\ref{eq:pw_2} mainly relies on the documents $\mc{D}_x$ (i.e. $\sum_{d \in \mc{D}_{x}}$), ignoring the social importance (or influence) of experts.
Our premise is that the expertise degree of $x$ on $t$ can depend not only on $x$'s knowledge on $t$, but also on $x$'s social importance among $t$'s collaborating experts in a given domain. Thus, we propose that an expert collaboration graph (i.e. \ecg) can also be a valuable source, in order to estimate such social importance. This estimation is achieved by identifying more \textit{authoritative} (or influential) {topic-sensitive experts} considering their joint documents. That is, in a sense, an \ecg is a social network for experts,
% and our idea is to reinforce the topic-sensitive weights of experts estimated by the $n$VSM with further experts' social importance (or influence) on the \ecg using \hits. 
% Thus, \EF collectively combines the weights of experts measured by considering associations between experts, documents and topics as well as  experts' authorities within the social community on the \ecg.
% We argue that an expert candidate's ex- pertise on a certain topic depends not only on whether the candidate has relevant knowledge, but also on the candidate's social importance or influence in the community. The idea is similar to what is behind a Web information retrieval technique [25], where the rank of a search result page with respect to a user query is determined by a combina- tion of content-based similarity and link-based importance.
% where RE(ca,q) denotes a relevance score between the documents (i.e., posts in online KCs) authored by the candidate ca and a user query q, AU(ca) denotes the global authority score of the candidate ca reflecting the social importance of the member within the community. The function f(•) is a combination strategy that collectively considers expertise relevance and authority to produce an expert ranking.
and \EF calculates the authority score of $x$ by repeatedly exploring the collective importance of the joint documents, published by $x$ and $x$'s coauthors, using \hits over the \ecg. More specifically, \EF incorporates the topic-sensitive weights of experts given topic, estimated by $n$VSM, into an \ecg and reinforces such weights using \hits.


% The key idea of \EF is to use a variation of HITS algorithm to further estimate the weights of experts for a given topic by integrating two knowledge facets: (1) the weights of experts and documents for a given topic estimated in $n$VSM; and (2) An expert collaboration graph (ECG) aims to express associations between experts and their documents using a directed, weighted bipartite graph.


% \definecolor{mywhite}{RGB}{255,255,255}
% \definecolor{myblue}{RGB}{0,0,255}
% \definecolor{mygreen}{RGB}{80,160,80}
% \definecolor{myblack}{RGB}{0,0,0}
% \definecolor{myred}{RGB}{255,0,0}
% \begin{figure*}[!h]
% \centering
% \begin{minipage}{.45\textwidth}
% \centering
% \begin{tikzpicture}[
%     node distance = 10mm and 40mm,
%     start chain = going below,
%     V/.style = {circle, draw, 
%                      fill=#1, 
%                      inner sep=0pt, minimum size=2mm,
%                      node contents={}},
%     every fit/.style = {ellipse, draw=#1, inner ysep=1mm, 
%                      inner xsep=5mm},
% ]

% % vertices 
% \foreach \i in {1,...,3} 
% {
%     \node (n1\i) [V=myblack,on chain,
%                   label={[text=myblack]left:$x_{\i}$}];
%     \node (n2\i) [V=myblack, right=22mm of n1\i,
%                   label={[text=myblack]right:$d_{\i}$}];
% \fi
% }
% % set U
% \node [myblack,fit=(n11) (n13),label=above:Experts ($\mc{X}$)] {};
% % set V
% \node [myblack,fit=(n21) (n23),label=above:Documents ($\mc{D}$)] {};
% % links
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm] (n11) edge[] (n21);
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm] (n11) edge[] (n22);
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm] (n12) edge[] (n21);
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm] (n12) edge[] (n22);
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm] (n12) edge[] (n23);
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm] (n13) edge[] (n23);
% \draw[<->, >=stealth', dashsed, shorten >=1mm, shorten <=1mm] (n11) edge[bend right=15, dashed] (n12);
% \draw[<->, >=stealth', dashsed, shorten >=1mm, shorten <=1mm] (n12) edge[bend right=15, dashed] (n13);
% \end{tikzpicture}
% \subcaption{(a)}\label{fig:ECG_a}
% \end{minipage}

% \begin{minipage}{.45\textwidth}
% \centering
% \begin{tikzpicture}[
%     node distance = 10mm and 40mm,
%     start chain = going below,
%     V/.style = {circle, draw, 
%                      fill=#1, 
%                      inner sep=0pt, minimum size=2mm,
%                      node contents={}},
%     every fit/.style = {ellipse, draw=#1, inner ysep=1mm, 
%                      inner xsep=5mm},
% ]

% % vertices 
% \foreach \i in {1,...,3} 
% {
%     \node (n1\i) [V=myblack,on chain,
%                   label={[text=myblack]left:$x_{\i}$},
%                   label={[text=myblue,shift={(0,0)}]:$A(x_{\i})$}];
%     \node (n2\i) [V=myblack, right=22mm of n1\i,
%                   label={[text=myblack]right:$d_{\i}$},
%                   label={[text=myred,shift={(0,0)}]:$H(d_{\i})$}];
% \fi
% }
% % set U
% \node [myblack,fit=(n11) (n13),label=above:Experts ($\mc{X}$)] {};
% % set V
% \node [myblack,fit=(n21) (n23),label=above:Documents ($\mc{D}$)] {};
% % links
% \draw[<-, >=stealth', shorten >=1mm, shorten <=1mm]
%         (n11) edge[bend right=10, dashed, red] (n21) 
%         (n11) edge[bend right=10, dashed, red] (n22)   
%         (n12) edge[bend right=10, dashed, red] (n21) 
%         (n12) edge[bend right=10, dashed, red] (n22) 
%         (n12) edge[bend right=10, dashed, red] (n23)
%         (n13) edge[bend right=10, dashed, red] (n23)
        
%         (n21) edge[bend right=10, dashed, blue] (n11) [left]
%         (n22) edge[bend right=10, dashed, blue] (n11)   
%         (n21) edge[bend right=10, dashed, blue] (n12) 
%         (n22) edge[bend right=10, dashed, blue] (n12) 
%         (n23) edge[bend right=10, dashed, blue] (n12)
%         (n23) edge[bend right=10, dashed, blue] (n13)
% \end{tikzpicture}
% \subcaption{(b)}\label{fig:ECG_b}
% \end{minipage}

% \caption{An example of the expert collaboration graph (ECG) and the score propagation of authority and hub nodes: (a) ECG's bipartite graph. The solid lines show associations between authorities (experts) and hubs (publications), and the dashed lines show collaboration relations between experts. (b) Iterative score propagation of authority and hub nodes. The blue dashed lines show the propagation of the authority scores of experts to publications. Also, the red dashed lines show the propagation of the hub scores of publications to experts.} \label{fig:ECG}
% \end{figure*}

Let ${G} = (V, E)$ be an \ecg (i.e. directed, weighted bipartite graph) that has two node types: experts $\mc{X}$ (also called \textit{authorities}) and documents $\mc{D}$ (also called \textit{hubs}). Thus, the node set $V$ = $\mc{X} \cup \mc{D}$.
In ${G}$, each expert is not connected to any other experts, and the same is with the documents. A directed edge points from a document $d \in \mc{D}$ to an expert $x \in \mc{X}$, if $x$ has the authorship on $d$. 
This edge is denoted as ${e_{dx}}$. 
Thus, the set of edges $E$ contain directed edges from $\mc{D}$ to $\mc{X}$. 
% There is no directed edge from $\mc{X}$ to $\mc{D}$. 
Given ${e_{dx}}$, its weight, denoted as $w_{dx}$, comes from $\mb{DX}_{i(d),i(x)}$ (see Section~\ref{sec:notation}). 
% As a value of $\mb{XD}_{x,d}$, in the simplest way, we can uniformly assign the same value, 1, to all the experts having the authorship on publication $d$, assuming that their weights on $d$ are the same. Another way is to consider the total number of the authors on $d$, assuming that all authors are equally important, that is, $\frac{1}{|\mc{X}_d|}$. Also, various heuristics can be used to infer this weight~\citep{Wang:2015}.

\begin{figure}[!h]
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \includegraphics[trim=0cm 0cm 0cm 0cm, width=100pt]{figures/graph_0.pdf}
        \subcaption{}
    \end{minipage}
    \quad
    \begin{minipage}[t]{0.45\linewidth}
        \centering
        \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=100pt]{figures/graph_1.pdf}
        \subcaption{}
    \end{minipage}  
    \caption{An example \ecg (a) and the score propagation of authority and hub nodes (b).}\label{fig:ECG}
\end{figure}

An example \ecg is depicted in Fig.~\ref{fig:ECG}(a), where the solid lines show associations between experts and documents. The dashed arrows show implicit collaborations between experts via their joint documents: e.g.,
% Each edge has its own weight indicating the relevance degree of an expert on a given document.
$x_1$ and $x_2$ have the joint documents $d_1$ and $d_2$, such that a collaboration between them is established as a bidirectional dashed arrow. 
% Another arrow exists between $x_2$ and $x_3$ due to the same notion. 
% We reinforce topic-sensitive weights of experts, measured in $n$VSM, by taking into account such implicit collaborations derived using \hits.

% In Fig.~\ref{fig:ECG} (b), we see iterative score propagation of authority and hub nodes. The blue dashed lines show the propagation of the authority scores (i.e. $A(x_1), A(x_2), A(x_3)$) of experts to documents. Also, the red lines show the propagation of the hub scores (i.e. $H(d_1), H(d_2), H(d_3)$) of documents to experts. The authority score, $A(x)$, estimates the importance of an expert $x$, and the hub score, $H(d)$ estimates the importance of a document $d$.


% For example, $x_1$ has the authorship in $d_1$ and $d_2$ with weights $\mb{XD}_{1,1}$ and $\mb{XD}_{1,2}$, respectively. 


\subsection{Reinforcing Expert Weights using \hits} \label{sec:cohits}
% \subsubsection{Hyperlink-Induced Topic Search (HITS) algorithm}\hspace*{\fill}

% The HITS algorithm is one of the page ranking algorithms used by search engines~\citep{Kleinberg:1999}. The basic idea behind HITS is that all web pages can be classified into two kinds: (1)  hubs and (2) authorities. Hubs can be defined as the web pages that have out-going links to other important web pages. Authorities can be defined as the web pages that have in-coming links from other important web pages. Thus, an important hub page is one that points to many important authorities; an important authority page is expected to be pointed to by many important hub pages. 
Note that \hits is a variation of CO-HITS~\citep{Hongbo:2009}. Thus, we first present the basic notion of CO-HITS on the structure of \ecg. That is, an important document is expected to point to important experts, while an important expert is linked by important documents. The importance of an expert $x$ is called the \textit{authority score} of $x$, and the importance of a document $d$ is called the \textit{hub score} of $d$. These scores are non-negative weights. Here, our goal is to reinforce the topic-sensitive weights of experts, estimated by $n$VSM, using \hits on the underlying \ecg.
% Thus, given the ECG, ${G} = (V, E)$, the authority score of an expert $x\in \mc{X}$ is denoted as $A(x)$, and the hub score of a publication $d \in \mc{D}$ as $H(d)$. 
% \subsubsection{Estimation of Authority Scores of Experts for Expertise Topics in ExpFinder}\label{sec:expfinder_algo}
% \hspace*{\fill}
% We now elaborate \EF's algorithm for estimating authority scores of expertise topics in the given ECG. 
For this, our idea is that given a topic $t$, we propagate the authority and hub scores with respect to $t$ by traversing $\mc{X}$ and $\mc{D}$ on the \ecg via an iterative process. 

An example is shown in Fig~\ref{fig:ECG}(b), 
% the experts will estimate their own authority scores (i.e. $A(x_1)$, $A(x_2)$, $A(x_3$) and the publications will estimate their own hub scores (i.e. $H(d_1)$, $H(d_2)$, $H(d_3$) based on an iterative process. 
where the hub scores, $H(d_1)$ and $H(d_2)$, are propagated to the expert $x_1$ to update the authority score $A(x_1)$; $H(d_2)$ is also propagate to update $A(x_2)$; and $H(d_3)$ is propagated to update $A(x_2)$ and $A(x_3)$. Once all the authority scores are updated, these scores are again propagated to the hubs to update their  scores. This performs iteratively. The intuition behind the iteration is the repeated mutual reinforcement to estimate authority and hub scores from co-linked nodes on the \ecg. 

In order for \EF to incorporate an topic into \hits, we take two steps. First, we extend the CO-HITS equation~\citep{Hongbo:2009} to accommodate a {topic}. We call this extension  \textit{topic-sensitive} CO-HITS. As the {initial authority and hub scores}, our {key idea } is to use the estimated topic-sensitive weights of experts and documents in $n$VSM, respectively. Second, we newly design and apply our variation of topic-sensitive CO-HITS into the \ecg. 
We elaborate these two steps in the rest of this section.

As the first step, we formally present the topic-sensitive CO-HITS equation, given an expert $x$ and a topic $t$:

% we extend Equation~\ref{eq:hits} in the way that incorporates expertise topics.
% Following the notation in the query-sensitive HITS equation~\citep{Daniel:2015}, we estimate the authority score of an expert $x \in \mc{X}$ given an expertise topic $t \in \mc{T}$ for $k$-th score propagation step of the generalised CO-HITS equation as follows: 
\begin{align}\label{eq:hits_topic}
    \begin{split}
    A(x;t)^k &= (1-\lambda_{x}) \alpha_{x;t} + \lambda_{x}\sum_{e_{dx} \in E} w_{dx} H(d;t)^{k-1} \\
    H(d;t)^k &= (1-\lambda_{d}) \alpha_{d;t} + \lambda_{d}\sum_{e_{du} \in E} w_{du} A(u;t)^{k}
    \end{split}
\end{align}
% \begin{align}
%     \begin{split}
%     A(x;t)^k &= (1-\lambda_{x}) A^{k-1}(x;t) + \lambda_{x}\sum w_{dx} H(d;t)^{k-1}, \\
%     H(d;t)^k &= (1-\lambda_{d}) H^{k-1}(d;t) + \lambda_{d}\sum w_{du} A(u;t)^{k},
%     \end{split}
% \end{align}\label{eq:hits_topic}
where 
\begin{itemize}
    \item $A(x;t)^k$ and $H(d;t)^k$ are the topic-sensitive authority score of $x$ and topic-sensitive hub score of $d$, respectively, given $t$ at $k$-th iteration. 
    % These scores indicate  topic-sensitive authority and topic-sensitive hub scores for $t$. 
    \item $w_{dx}$ denotes the weight of the edge $e_{dx}$, and thus  $w_{dx}=\mb{DX}_{i(d),i(x)}$ and $w_{du} = \mb{DX}_{i(d),i(u)}$, where $i(d)$ and $i(x)$ indicate the row and column index of $d$ and $x$, respectively, on $\mb{DX}$.
    \item $k$ indicates a iteration number staring from 1.
    \item $\alpha_{x;t}$ is the initial score for $A(x;t)^*$ and $\alpha_{d;t}$ is the initial score for $H(d;t)^*$ given $t$. 
    We call these scores \textit{personalised weights}.
    In this work, these personalised weights are normalised to be the widely used L2-norm~\cite{Kleinberg:1999}, that is, $\left(\sum_{x_i\in \mc{X}}
    \alpha_{x_i;t}\right)^{1/2}$ = $1$ and $\left(\sum_{d_i\in \mc{D}}
    \alpha_{d_i;t}\right)^{1/2}$ = $1$. Also, after updating the $k$-th iteration, the square root of the sum of squares of $A(x;t)^k$ and $H(d;t)^k$ are normalised using L2-norm, respectively. 
    % Note that $H(d;t)^0$ is equal to  $\alpha_{d_i;t}$. 
    Assigning the personalised weights provides crucial information in CO-HITS as they provide valuable and make an impact on the propagation of the updates of both authority and hub scores~\cite{Hongbo:2009}. 
    Our approach to determining the personalised weights is presented when discussing our proposed variation equation of Eq.~\ref{eq:hits_topic2}.
    
    % In our approach, $A(x)_t^0$ and $H(d)_t^0$ are given as $\mb{TX}_{i(t),i(x)}$ and $\mb{TD}_{i(t),i(d)}$ respectively. 
    
    % Note that $\mb{TX}_{i(t),i(x)}$ indicates the  weight of $x$, and $\mb{TD}_{i(t),i(d)}$ is the weight $d\in \mc{D}_x$ for $t$, that have been estimated in the $n$VSM.
    \item $\lambda_{x}\in [0,1]$ and $\lambda_{d} \in [0,1]$  are  \textit{personalised parameter} for expert and document, respectively. These parameters determine how much we consider the personalised weights when calculating the $k$-th scores. Assigning lower values  indicates that higher importance is given to the personalised weights while reducing the propagation effects of co-linked nodes.
    
    % \item $\lambda_{x}\in [0,1]$ and $\lambda_{d} \in [0,1]$  are called \textit{personalised parameter} for expert and document, respectively. These parameters determine how much we consider the ($k$-1)-th authority and hub scores when calculating the $k$-th scores. Assigning lower values of these parameters indicates that higher importance is given to the initial scores while reducing the propagation effects of co-linked nodes.
    \item Using Eq.~\ref{eq:hits_topic}, the topic-sensitive CO-HITS algorithm performs as follows: (1) with the personalised weights, a user-specified $k$ and a topic $t$, update all authority scores of $\mc{X}$; and (2) update all hub scores of $\mc{D}$. These steps are repeatedly performed $k$ times.
\end{itemize}


% Also, in the same way, $\delta_{x;t}$ and $\delta_{d;t}$ denote the personalised weight of $x$ and $d$,  respectively, given $t$.
% Thus, we denote consider a given expertise topic $t$ to estimate the authority score $A(x)$ of each expert $x$ using the above intuition. 

% The personalised weight for an expert denotes a weight in relation to the other experts determined by prior knowledge about the experts in $\mc{X}$, and the sum of the personalised weights for all the experts in $\mc{X}$ is equal to 1, that is, $\sum_{i=1}^{|\mc{X}|} \delta_{x_i}=1$. Similarity, the personalised weight for a publication denotes a weight in relation of the other publications determined by prior knowledge about publications in $\mc{D}$, and $\sum_{i=1}^{|\mc{D}|} \delta_{d_i}=1$. The initial values (i.e. at the 1-th propagation step) of the personalised weights for both experts and publications are given priori based on a certain criteria. For the $k$-th propagation steps ($K > 1$), the personalised weights for experts and publications weights are determined by $A(x)^{k-1}$ and $H(d)^{k-1}$, respectively.

In the second step, we design the \hits equation and apply it on the underlying \ecg using two variation schemes of topic-sensitive CO-HITS:

\begin{equation}\label{eq:hits_topic2}
\scalemath{0.92}{
    \begin{split}
        A(x;t)^k &= (1-\lambda_{x}) A(x;t)^{k-1} + \lambda_{x}\left(\frac{\sum\limits_{e_{dx} \in E} w_{dx} H(d;t)^{k-1}}{\sum\limits_{e_{dx} \in E} w_{dx}} \right) \\
        H(d;t)^k &= (1-\lambda_{d}) H(d;t)^{k-1} + \lambda_{d} \left(\frac{\sum\limits_{e_{du} \in E} w_{du} A(u;t)^{k}}{\sum\limits_{e_{du} \in E} w_{du}} \right)
    \end{split}
}
\end{equation}
% \begin{align}
%     \begin{split}
%     A(x;t)^k &= (1-\lambda_{x}) A^{k-1}(x;t) + \lambda_{x}\sum w_{dx} H(d;t)^{k-1}, \\
%     H(d;t)^k &= (1-\lambda_{d}) H^{k-1}(d;t) + \lambda_{d}\sum w_{du} A(u;t)^{k},
%     \end{split}
% \end{align}\label{eq:hits_topic}

where the interpretation of all the variables is the same as presented for Eq.~\ref{eq:hits_topic}, except the following two variation schemes. 

The first variation scheme is that rather than using the \textit{fixed} personalised weights $\alpha_{x;t}$ and $\alpha_{d;t}$, \hits uses \textit{dynamic} personalised weights $A(x;t)^{k-1}$ and $H(d;t)^{k-1}$ at each $k$-th iteration. In Eq.~\ref{eq:hits_topic}, regardless of iterations, the authority and hub scores at each iteration are fixed to be $\alpha_{x;t}$ and $\alpha_{d;t}$. Different from it, our approach is to use personalised weights at the $k$-th iteration as the ($k$-1)-th authority and hub scores. By doing so, in the calculation of the authority (resp. hub)  scores at the $k$-th iteration, the our aim is to exploit 
both the propagation of the hub (resp. authority) scores and the effect of the authority (resp. hub) score at the ($k$-1)-th iteration. 
% Thus, there can be a high tendency that topic-specific CO-HITS ignores how the propagation of the authority and hub scores at the ($k$-1)-th iteration can incrementally impact on the calculation of the personalised weights at the $k$-th iteration.
Thus, in \hits, personalised weights are updated at each iteration based on the authority and hub scores at the previous iteration. In our approach, as the initial personalised weights, we use the topic-sensitive weights of experts and documents estimated using $n$TFIDF in $n$VSM. Thus, $A(x;t)^{0}$ = $\mb{TX}_{i(t),i(x)}$ and $H(d;t)^{0}$ = $\mb{TD}_{i(t),i(d)}$.
Similarly, in the topic-sensitive CO-HITS equation in Eq.~\ref{eq:hits_topic}, $\alpha_{x;t}$ and $\alpha_{d;t}$ are set to be $A(x;t)^{0}$ and $H(d;t)^{0}$, respectively.
By doing so, we integrate $n$VSM  with \hits, generating a new unified formula for this integration. Our intuition for this integration is to improve
the accuracy for expert finding by further exploring the implicit relationships between experts, derived from the \ecg, in addition to the results of the $n$VSM approach. Note that $n$VSM  ignores such relationships, only utilising the importance of a document $d$; the importance of a topic $t$ from the documents of an expert $x$; and the importance of $x$ given $d$ (see Eq.~\ref{eq:pw_2}).
    
The second variation scheme is that the \textit{aggregation} of the authority and hub scores is different from that of topic-sensitive CO-HITS. In Eq.~\ref{eq:hits_topic}, $A(x;t)^{k}$ and $H(d;t)^{k}$  are calculated based on the square root of the \textit{sum} of squares of $H(d;t)^{k-1}$ and $A(x;t)^{k}$, respectively. This approach tends to assign a higher authority score to an expert $x$ who has \textit{more} documents (i.e. $|\mc{D}_x|$). Similarly, it is likely that a higher hub score is given  to a document $d$ that is linked to \textit{more} experts (i.e. $|\mc{X}_d|$) that have $d$.

Instead, in \hits, we use the \textit{central tendency} of $H(d;t)^{k-1}$ to calculate $A(x;t)^{k}$; and also use the \textit{central tendency} of $A(x;t)^{k}$ to calculate $H(d;t)^{k}$. The `average' is used to measure such central tendency. The  reason is that we have already incorporated the idea of using `the sum of squares of authority and hub scores', used in topic-sensitive CO-HITS, in the context of $n$VSM. Note that in $n$VSM, we calculated the topic-sensitive weights of experts by using the \textit{sum} operator as seen in Eq.~\ref{eq:pw_2} (i.e. $\sum_{d \in \mc{D}_{x}}$). Thus, to avoid the duplicated use of this `sum' operator, given a topic $t$, we design \hits in a way that estimates the importance of an expert $x$ at the $k$-th iteration (i.e. $A(x;t)^k$) by calculating the \textit{average} of the ($k$-1)-th hub scores, in addition to personalised weight $A(x;t)^{k-1}$. Similarly, we estimate the importance of a document $d$ (i.e. $H(d;t)^k$) by calculating the \textit{average} of the $k$-th authority scores, in addition to personalised weight $H(d;t)^{k-1}$. In the name \hits, `$\mu$' indicates the `average' so that \hits means a particular topic-specific CO-HITS using the 'average' importance of authority and hub scores.

We also highlight other features of \hits. First, as with  topic-sensitive CO-HITS, the updated authority and hub scores at each iteration are normalised using L2-norm.
Second, if $\lambda_x$ and $\lambda_d$ are 0, \hits returns the initial personalised weights at each iteration. Thus, \EF does not use the score propagation effects on the \ecg, returning the same results obtained from $n$VSM. Third, if $\lambda_x$ and $\lambda_d$ are all equal to 1, \hits does not incorporate personalised weights. However, it calculates $H(x;t)^{1}$ based on the $H(d;t)^{0}$ that was obtained from the topic-document matrix $\mb{TD}$, i.e.,  $H(d;t)^{0}$ = $\mb{TD}_{i(t),i(d)}$, generated by $n$VSM. Also, $H(d;t)^{1}$ is calculated based on $A(u;t)^{1}$.

% \EF differs from the work \citep{Daniel:2015} in estimating the personalised weights in the equation: First, the work~\citep{Daniel:2015} defines the personalised weight of an organisation based on the simple notion of how many projects are related to a given topic each year, assuming that such frequency information is available and manually given. Instead, \EF does not require such information and automatically defines the personalised weights of experts based on a language model that takes into account a probability distribution over sequences of words. Second, the work~\citep{Daniel:2015} uses the personalised weight of a project based on how much funding it receives over the total amount of the funding assigned to all underlying projects within the target domain. However, a limitation of this weighting scheme is that it is not topic-sensitive as topic information is not incorporated into the estimation of this weight. However, \EF incorporates topic information into the estimation of the personalised weight of each publication based on its importance over a given expertise topic. Consequently, \EF is a hybrid method that incorporate (1) rigorous semantics analysis of expertise topics given publications using a language model into (2) the topic-sensitive HITS algorithm to boost the two knowledge facets together in a unified manner. 
 


% {\bf Estimation of personalised weights for publications.}

% The personalised weight of  a publication $d$ with respect to an expertise topic $t$ is denoted as $p(d|x)$ and driven by:
% \begin{equation}\label{eq:pw_pub}
%     p(d|t) = p(t) * p(t|\theta_d)
% \end{equation}

% In Equation~\ref{eq:pw_pub}, $p(t|d)$ is calculating using Equation~\ref{eq:document_model}, and $p(t)$ is equal to $p(t|\mc{D})$ that is estimated as the average value of the $t$-th column values $\vec{\mb{DT}}_{*,t}$ in $\mb{DT}$.

%This value can be estimated by considering semantic information of $t_i$ in a given domain knowledge, if provided. Often such domain knowledge can be provided in the form of an taxonomy~\cite{Kang:2016}. A taxonomy describes domain-specific topics (or concepts) and relationships among them in a hierarchy. We can infer an importance of each topic by estimating its semantic by navigating the hierarchical relationships between that topic and the others in the taxonomy. Intuitively, in a taxonomy, the lowers topics have more weights than the higher topics. Because the lower topics inherit all the characteristics from their superordinate topics. The higher the position of a topic in a taxonomy, the more abstract the topic is. As an example of the weight of $tw_1$, we can use the measure estimating the information content of topic $t_i$ in a given taxonomy using the information content-based approach~\cite{Seco:2004}.

% We argue that an expert candidate's ex- pertise on a certain topic depends not only on whether the candidate has relevant knowledge, but also on the candidate's social importance or influence in the community. The idea is similar to what is behind a Web information retrieval technique [25], where the rank of a search result page with respect to a user query is determined by a combina- tion of content-based similarity and link-based importance.

% where RE(ca,q) denotes a relevance score between the documents (i.e., posts in online KCs) authored by the candidate ca and a user query q, AU(ca) denotes the global authority score of the candidate ca reflecting the social importance of the member within the community. The function f(•) is a combination strategy that collectively considers expertise relevance and authority to produce an expert ranking.


==> Expertise Retrieval_TKDE/eval_result.tex <==
\section{Evaluation of \EF}\label{sec:eval}
To assess the effectiveness of \EF, we conduct the following evaluation. First, we measure the effectiveness of the first knowledge facet of \EF: $n$VSM (Section~\ref{sec:weight_eval}).
% ., in comparison with with TFIDF-based VSM and two DLM-based approaches~\cite{Balog:2009,Wang:2015,WISER:2019} (Section~\ref{sec:weight_eval}). 
Second, we show how to empirically find the best values for personalised parameters of \EF (Section~\ref{sec:lamb_eval}). 
Third, we evaluate that \EF is a highly competitive model for expert finding, in comparison with $n$VSM and the two GM approaches~\citep{Gollapalli:2013,Daniel:2015}. Further, to show the capability of the second knowledge facet of \EF, i.e., \hits, over topic-sensitive CO-HITS (simply CO-HITS), we compare \EF with an alternative \EF form that combines $n$VSM and CO-HITS (Section~\ref{sec:eval_ef}). Finally, we summarise our evaluation (Section~\ref{sec:discussion}).

\subsection{Datasets}\label{sec:data}
% \amir{It would be great to summarise the number of #Documents, #Topics and #Experts. The total numbers represent the overall scope of the study, and it would be great to also repeat this in the Conclusion. }

We use four benchmark datasets in our evaluation. One is the {Lattes Expertise Retrieval} ({{\textit{LExR}}})\footnote{LExR is available to download from \url{http://toinebogers.com/?page_id=240}} test collection~\citep{Vitor:2016} for expertise retrieval in academic. LExR provides a comprehensive, large-scale benchmark for evaluating expertise retrieval and it covers all knowledge areas (e.g. earth sciences, biology, health sciences, languages, art, etc) working in research institutions all over Brazil. Most publications are written in Portuguese, Spanish and English. In our evaluation, we only consider the English documents for our readability. 
% Each publication contains information about authors, published year, keywords, research areas, abstract and title. 
The other three datasets\footnote{These datasets can be downloaded from  \url{http://www.lbd.dcc.ufmg.br/lbd/collections}.} are Information Retrieval (IR), Semantic Web (SW), and Computational Linguistics (CL) which are filtered subsets of DBLP dataset \citep{bordea2013benchmarking}. 
% Each publication contains authors, published year, published venues, citations, abstract and body-text. 
In these four datasets, we regard the authors as experts $\mc{X}$ and the publications as documents $\mc{D}$, where each publication is seen as a mixture of title and abstract. From $\mc{D}$, we extract phrases as the first step in \EF (Section~\ref{sec:overview}). 

These datasets also provide the ground-truth about who are the known experts for the  known topics. The expert degrees for each topic are represented as non-relevance, relevance, and high relevance in LExR. We regard individuals with non-relevance as \textit{non-experts}, and individuals with relevance and high relevance as \textit{experts}.
IR, SW and CL also provide the expert list for each topic. We formalise the candidates in such list as \textit{experts}, and otherwise \textit{non-experts}.

% There are also three different ground truth collections related to three areas - Information Retrieval (IR), Semantic Web (SW), and Computational Linguistics (CL). Each ground truth collection is in XML format where each entry contains a workshop information with its id, expertise topics, organisers and program committees (experts). Unlike the IR collection containing experts with their associated id, SW and CL collections do not contain associated id for each expert. Due to the absence of relevancy score in three ground-truth datasets, we assigned a default relevancy of 1 to all author-topic associations for each dataset.
% Each author associates with an id. There is also a ground-truth dataset for expert finding. The dataset is provided with the mapping of author id with listed 233 topics. Each entry also contains a relevancy score such as non-relevance (0), relevance (1), or high relevance (2).
% LexR contains publications collected from journals, conference papers or book chapters of a number of experts invovled in various research activities in Brazil such as earth sciences, biology, health sciences, languages and others. Each entry contains some basic information about the publication such as authors, published year, keywords, research areas, abstract and title. Each author associates with an id. There is also a ground-truth dataset for expert finding. The dataset is provided with the mapping of author id with listed 233 topics. Each entry also contains a relevancy score such as non-relevance (0), relevance (1), or high relevance (2).
% The domain-specific expert search collection contains a filtered version of DBLP dataset in XML format where each entry contains a document with its id, title, list of authors, published year, venues, number of citations, abstract and text containing the entire content. Each author associates with an id. There are also three different ground truth collections related to three areas - Information Retrieval (IR), Semantic Web (SW), and Computational Linguistics (CL). Each ground truth collection is in XML format where each entry contains a workshop information with its id, expertise topics, organisers and program committees (experts). Unlike the IR collection containing experts with their associated id, SW and CL collections do not contain associated id for each expert. Due to the absence of relevancy score in three ground-truth datasets, we assigned a default relevancy of 1 to all author-topic associations for each dataset.
From each dataset, we preprocess the following steps to be used in our evaluation. First, we remove publications containing empty title and abstract. Second, we remove publications whose abstracts provide little information, that is, less than 5 words after removing stopwords. 
Third, if there exists duplicated topics, we remove such ones.
Table \ref{tab:data_desc} shows an overview of the datasets after performing these steps.

\captionsetup[table]{labelfont=bf, skip=0pt}
\begin{table}[!h]
    \caption{A summary of our four datasets}
    \begin{center}
        \scalebox{0.87}{
            \setlength{\tabcolsep}{4pt}
            \begin{tabular}{p{5cm}rrrr}
            \hline
            & LExR & IR & SW & CL \\
            \hline
            \# of documents & 14879 & 2355 & 1519 & 1667 \\
            \# of experts & 620 & 276 & 394 & 358 \\
            \# of topics & 227 & 268 & 2046 & 1583 \\
            Avg. \# of documents per expert & 28 & 9 & 4 & 5 \\
            % Avg. \# of topics per expert & 2 & 10 & 46 & 36 \\
            Avg. \# of experts per topic & 6 & 10 & 9 & 8 \\
            Median \# of experts per topic & 5  & 8 & 6 & 5 \\
            % Min \# of experts per topic & 1  & 1 & 1 & 1 \\
            Max \# of experts per topic & 26  & 177 & 226 & 158 \\
            % Std \# of experts per topic & 4 & 12 & 12 & 12 \\
            \hline
            \end{tabular}
        }
    \end{center}
    \label{tab:data_desc}
% \vspace{-10pt}
\end{table}

We note that our chosen datasets are relatively more comprehensive than some previous works, which focused on academic domains for their evaluation, in terms of the number of topics considered, thereby providing a reasonable measure of the effectiveness of \EF. For example, the works \cite{Deng:2008}, \cite{Gollapalli:2013} and \cite{Wang:2015} used two datasets with seven topics, two datasets with 13 and 203 topics and one dataset with 14 topics, respectively\footnote{These datasets are also no longer publicly available.}. Note that our evaluation
have been done using the larger numbers of the topics on the four datasets as seen in Table~\ref{tab:data_desc}.




\begin{table*}[!t]
    \caption{Expertise topics and corresponding similar phrases in four datasets}
    \begin{center}\label{tab:sim_pt}
        \scalebox{0.6}{
            \begin{tabular}{cc|cc|cc|cc}
            \toprule
            \multicolumn{2}{c}{LExR} & \multicolumn{2}{c}{IR}  & \multicolumn{2}{c}{SW}  & \multicolumn{2}{c}{CL} \\
            \cmidrule{1-8}
            Topic & Phrase & Topic & Phrase & Topic & Phrase & Topic & Phrase \\
            \midrule
            synthesis & synthesis & information retrieval & information retrieval & semantic web & semantic web & question answering & question answering  \\
            risk factor & risk factor &  search engine & search engine & linked data & linked data & knowledge transfer & knowledge transfer \\
            public health & public health & patent search & patent search & text understanding & text understanding & summarization & summarization \\
            thin film & ultrathin film & data modelling & information modelling & auction & bidding & machine vision & computer vision \\
            development validation & validation process & cooperative work & collaborative working & invalidity & inadequacy & image classification & image recognition \\
            \bottomrule
            \end{tabular}            
        }
    \end{center}
\vspace{-10pt}
\end{table*}
% \vspace{-4pt}
% \begin{enumerate}
%     \item We removed entries that contains missing values in both collections. Importantly, we kept entries that contains non-empty title and abstract.
%     \item We merged the title and abstract fields into one field, so-called the text field, separating by a dot and space.
%     \item We removed existing stop words in the text field and then selected entries with text containing more than or equal to 5 words.
%     \item To construct a list of expertise topics for IR, CL and SW datasets, we extracted those from the XML structure and sequentially assigned a unique id for each topic. Note that the LExR collection contains the processed ground-truth dataset in the proper format.
%     \item We removed duplicate expertise topics.
%     \item Using the processed collection in Step 3 for IR, SW and CL datasets, we selected experts for the IR ground-truth dataset based on their unique ids. Meanwhile, we used experts' full name to select them for SW and CL ground-truth datasets and extracted their ids from the collection.
%     \item For IR, SW and CL datasets, we mapped expertise topics to experts via experts' id and assigned default relevancy score of 1 to each expert-topic association.
%     \item For both collections, we used experts' ids in each ground-truth dataset to filter number of documents.
% \end{enumerate}

% \captionsetup[table]{labelfont=bf, skip=0pt}


\subsection{Evaluation Framework}\label{sec:eval_frame}
We present our evaluation configuration and metrics. Recall that as a topic, we use a phrase. We assume that the maximum word length of each phrase is 3 in our evaluation. Also, we observe that there is no guarantee that an original known topic $t_g$ always appears in documents $\mc{D}$ in each dataset. 
Thus, given each $t_g$, we find its most similar phrase $t$ from $\mc{D}$. Then, $t$ is alternatively used as a topic, instead of $t_g$.
To find $t$ given $t_g$, we use the scientific pre-trained model SciBERT\footnote{The pre-trained SciBERT model can be downloaded at \url{https://github.com/allenai/scibert}}~\citep{Beltagy2019SciBERT} that is a scientific language model trained on the fulltext of 1.14M papers and 3.1B words, where the papers were collected from `semanticscholar.org'.
Using this model allows us to measure a semantic similarity between $t_g$ and $t$ by their cosine similarity according to their corresponding vectors represented in the model. More specifically, assume that $s_1$ is an original known topic and $s_2$ is a phrase extracted from $\mc{D}$. Then, we measure their similarity as:

\begin{equation}
    sim(s_1, s_2) \approx \cos(\vec{s_{1}}, \vec{s_{2}}) = \frac{\vec{s_{1}}^{\,} \cdot \vec{s_{2}}^{\,} }{\left\Vert \vec{s_{1}}^{\,} \right\Vert \left\Vert \vec{s_{2}}^{\,} \right\Vert},
\end{equation}
where $\vec{s_1}$ and $\vec{s_2}$ are the represented vectors of $s_1$ and $s_2$ in SciBERT, respectively. Each of these vectors is estimated by the average of the embedded vectors of its constituent terms. 
Suppose that $s_1$ consists of $n$-terms, $s_1 = (w_1, \ldots, w_n)$, then,
$\vec{s_1} \approx \frac{1}{n} (\vec{w_1} + \ldots + \vec{w_n}),$
where $(\vec{w}_1, \ldots, \vec{w}_n)$ are the embedded vectors of $(w_1, \ldots, w_n)$. The same principle is applied to $s_2$. Table~\ref{tab:sim_pt} shows the  examples of five topic-phrase pairs  in each dataset, where each pair shows an original known topic $t_g$ and the most similar phrase $t$ used as a topic in our evaluation. As we see, some phrases ($t$) are equal to the original topic ($t_g$), while some others phrases are semantically very similar to the corresponding original topic (e.g. `image classification'-`image recognition' on CL).
% Finally, for each original topic name $t_g$, we identify the most similar phrase $t$ and use it as an alternative topic name using the above euqation.

Other evaluation configuration includes: (1) we assume that the importance of documents is the same (i.e. $p(d)$=1) and the importance of all experts of $d$ is the same (i.e. $p(x|d)$=1) in Eq.~\ref{eq:pw_2}. The reason is that one of our primary focuses is to evaluate the capability of $n$TFIDF in $n$VSM in calculating $p(t|d)$ in Eq.~\ref{eq:pw_2};
% and compare it with the DLMs~\cite{Balog:2009,Wang:2015,WISER:2019} and the TFIDF-based VSM; 
(2) Thus, we also fix $w_{dx}$=1 and $w_{du}$=1 in Eq.~\ref{eq:hits_topic} and Eq.~\ref{eq:hits_topic2}; and (3) from our empirical testing, we observed Eq. \ref{eq:hits_topic} and Eq. \ref{eq:hits_topic2} are commonly converged after 5 iterations, so we set $k = 5$.
% and (4) In Eq. \ref{eq:ntfidf}, we ignore a phrase with a negative $nidf$ value as such a value indicates that the phrase is not meaningful~\citep{nidf:2017}.


% \subsection{Evaluation Metrics}
For all expert finding models in our evaluation, our aim is to generate a ranked list of experts based on the outcome of the formula: (1) Eq.~\ref{eq:hits_topic2} in \EF, (2) Eq.~\ref{eq:hits_topic} in CO-HITS, (3) Eq.~\ref{eq:pw_2} and Eq.~\ref{eq:topic_by_terms} in DLM, (4) Eq.~\ref{eq:pw_2} and Eq.~\ref{eq:entropy2} in TFIDF-based VSM,  and (5) Eq.~\ref{eq:pw_2} and Eq.~\ref{eq:ntfidf} in $n$VSM, where all these methods are compared, in addition to WISER~\cite{WISER:2019} and RepModel~\cite{Daniel:2015}.

We use two widely-used evaluation metrics for expert finding~\citep{Wang:2015, Hongbo:2009}:
% \citep{Wang:2015, Hongbo:2009, Deng:2008}:  
(1) {\it precision at rank n (P@n)} and (2) {\it Mean Average Precision (MAP)}. P@n measures the relevance of the $n$-top ranked experts with respect to a given query topic, defined as~\citep{Hongbo:2009}:
\begin{equation}
    P@n = {
    |S_{n} \cap R_{t}|
    }/{n},
    % P@n = \frac{
    % |S_{n} \cap R_{t}|
    % }{n},
\end{equation}
where $S_{n}$ is the set of $n$-top recommended experts for a given topic $t$, and $R_{t}$ is the set of known experts for $t$. We report from P@10 to P@30 (increasing by 5) for each topic and take the average over all topics. MAP measures the overall ability of a method to differentiate between known experts and non-experts. The \textit{average precision (AP)} is defined as~\citep{Wang:2015}:
\begin{equation}\label{eq:AP}
    AP = \frac{
    \sum_{i=1}^{n}(P@i * rel(i))
    }{|R_{t}|}
\end{equation}
where $i$ is the rank, $rel(i)$ is a binary function indicating 1, if the result at $i$ is a known expert, otherwise 0. MAP is the mean value of AP values over all topics, and we use $n = 30$ as used in~\cite{Deng:2008}.



\begin{figure*}[!t]
\begin{center}
    \begin{tabular}{llll}
      \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/CLExR.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/CIR.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/CSW.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/CCL.pdf}
    \end{tabular}
    \caption{Comparison on the average precision (AP) values: x-axis shows n of P@n and y-axis shows AP values.}
    \label{tab:eval_APC}
\end{center}
\end{figure*}


\captionsetup[table]{labelfont=bf, skip=0pt}
\begin{table*}[!t]
    \caption{MAP and the the improvement ratio of $n$VSM.}
    \begin{center}
        \scalebox{0.9}{
            \setlength{\tabcolsep}{9pt}
            \begin{tabular}{l r l r l r l r l r l}
            \hline
            & LExR & & IR & &  SW & & CL & & Avg. \\
            \hline
            DLM-0.5 & 0.200 & (233.0\%) & 0.208 & (6.7\%) & 0.070 & (51.4\%) & 0.063 & (68.3\%) & 0.135 & (103.7\%) \\
            DLM-0.6 & 0.159 & (318.9\%) & 0.185 & (7.8\%) & 0.068 & (55.9\%) & 0.058 & (82.8\%)  & 0.118 & (133.1\%) \\
            TFIDF & 0.493 & (35.1\%) & 0.206 & (7.8\%) & 0.087 & (21.8\%) & \textbf{0.120} & (-11.7\%) & 0.226 & (21.7\%) \\
            WISER & 0.117 & (469.2\%) & 0.150 & (48.0\%) & 0.057 & (86.0\%) & 0.051 & (107.8\%) & 0.094 & (192.6\%) \\
            $n$VSM & \textbf{0.666} &  & \textbf{0.222} & & \textbf{0.106} &  & 0.106 &  & \textbf{0.275} & \\
            \hline
            \end{tabular}
        }
    \end{center}
    \label{tab:eval_MAPC}
\vspace{-10pt}
\end{table*}

\subsection{Evaluation of $n$VSM} \label{sec:weight_eval}
As $n$VSM is one key compoenent in \EF, we first measure its effectiveness. As presented in Section~\ref{sec:ntfidf}, the concepts VSM and DLM are closely related. Thus, we compare $n$VSM with TFIDF-based VSM and two particular DLMs:
% In Section~\ref{sec:eval_ef}, we will evaluate \EF over other GMs. Here, we compare $n$VSM with the three models: 
(1)
% the DLM approach is represented using Eq.~\ref{eq:pw_2} and Eq.~\ref{eq:topic_by_terms}. The TFIDF approach is represented using Eq.~\ref{eq:pw_2} and Eq.~\ref{eq:topic_by_terms}.
\textit{{TFIDF}-based VSM} expressed using Eq.~\ref{eq:pw_2} and Eq. \ref{eq:entropy2} (denoted as TFIDF); (2) \textit{The {DLM} model}~\citep{Balog:2009,Wang:2015} denoted using Eq.~\ref{eq:pw_2} and Eq.~\ref{eq:topic_by_terms} in which the probability of individual terms is estimated by Eq.~\ref{eq:document_model}, where we use two values for the best $\lambda_\theta$: 0.5 (\textit{DLM-0.5}) and 0.6 (\textit{DLM-0.6}), as suggested by \citep{Balog:2009} and \citep{Wang:2015}, respectively; and
(3) A recent probabilistic model {\textit{WISER}}~\cite{WISER:2019} that combines the document-centric approach exploiting the occurrence of topics in experts' documents, with the profile-centric approach computing relatedness between experts using an external knowledge source, Wikipedia. Since our work does not consider such an external knowledge source, we only consider WISER with the document-centric approach for the fair comparison. In WISER,
the topic-sensitive weight of an expert $x$ given a topic $t$ is calculated using Reciprocal Rank~\cite{Macdonald:2006}: $\sum_{d}^{\mc{D}_{x, t}}$ $\frac{1}{rank(d)}$ that represents the ranks of $x$'s documents where $t$ appears ($\mc{D}_{x, t}$). Since $t$ is a phrase, $\mc{D}_{x, t}$ consists of the subset of $\mc{D}_x$ that any of $t$'s constituent terms appears. $rank(d)$ is the ranking position of a document $d$ out of $\mc{D}$, where the position is determined by BM25~\citep{BM25:2009}. The hyper-parameters $k1$ and $b$ in BM25 are set to be 1.2 and 0.75, respectively, based on the suggestion~\cite{Yuanhua:2011}. 

The evaluation results are presented in Fig. \ref{tab:eval_APC} that
% \amir{Average precision less than 0.2 seems to be very low. Is this correct?} 
shows the AP values with n (n=10, 15, $\ldots$, 30) of P@n for all topics. We observe the following: (1) Overall, the VSM approaches (TFIDF and $n$VSM) largely outperform all DLM-0.5, DLM-0.6 and WISER. This  indicates the VSM approaches can be more effectively used for identifying topic-sensitive experts than the compared DLMs; (2) DLM-0.5 is consistently better than DLM-0.6 but their difference seems minor; and (3) $n$VSM is clearly better than TFIDF from P@10 to P@30 consistently over all the four datasets. Also, $n$VSM substantially outperforms all the compared methods on all the four datasets. 
% This proves that the proposed $n$VSM is a competative approach for expert finding outperforming the TFIDF-based VSM as well as the DLM approach. Also, this shows that \EF is equipped with a powerful component (the $n$VSM) for expert finding.
% We now evaluate $n$VSM in MAP. 
Table \ref{tab:eval_MAPC} shows the results on MAP and the relative improvement ratio of $n$VSM over the other models. The best one in each dataset is denoted in boldface. We see that $n$VSM's improvements over DLM-0.5 and DLM-0.6 are substantial: up to 318.9\% over DLM-0.6 on LExR, 7.8\% over DLM-0.6 on IR, 55.9\% on CL, and 82.8\% on CL. Moreover, $n$VSM substantially outperforms WISER from 48.0\% on IR to 469.2\% on LExR. Also, $n$VSM is highly better than TFIDF except the only one case on CL.
On average, we observe that $n$VSM largely outperforms DLM-0.5 in 103.7\%; DLM-0.6 in 133.1\%; WISER in 192.6\%; and TFIDF in 21.7\% across the four datasets. 
% In summary, we see that $n$VSM performs very well and achieves outperformance than the compared methods. 
In summary, the results show an empirical evidence that $n$VSM can be competitive and effectively used for expert finding. Also, these show that \EF is equipped with a powerful component, $n$VSM, for expert finding.

% \yb{add 0.2 is acceptable}

\subsection{Finding the Best Values for Personalised Parameters in \EF: $\lambda_x$ and $\lambda_d$} \label{sec:lamb_eval}
We now present how to empirically find the best values for personalised parameters  $\lambda_{x}$ and $\lambda_{d}$ of \hits (see Eq.~\ref{eq:hits_topic2}) which is another key component of \EF. Our approach is to make a full use of all the four datasets to determine such values. For this, we measure the \textit{mean} impact of different values of $\lambda_{x}$ and $\lambda_{d}$, respectively, on generating the MAP results from the four datasets. Our aim is to provide an empirical guideline for choosing the best values for these parameters. 
Formally, let $Z$ be the set of candidate values [0, 0.1, $\ldots$, 1.0] for $\lambda_{x}$ and $\lambda_{d}$. Then, let us define MAP$(a, b)$ as the MAP value using a pair of $a\in Z$ for $\lambda_{x}$ and $b\in Z$ for $\lambda_{d}$. 
First, we choose the best value for $\lambda_{x}$. To this end, for each value $a \in Z$, we compute the mean of the MAP values with all values in $Z$ in each dataset:

\begin{equation}\label{eq:avg_lambda_x}
Avg(a, \lambda_{x}) = \frac{1}{|Z|}\sum_{b \in Z}{\textrm {MAP}} (a, b).
\end{equation}
Then, we obtain the $|Z|$-length vector of $Avg(a, \lambda_{x})$ for all values in $Z$. Let us say that this vector is denoted as $Avg(Z, \lambda_x)$. For example, if $Avg(Z, \lambda_x) = [1, 0.9, 0.8, \ldots, 0]$, then the corresponding element-wise rank vector is $R(Avg(Z, \lambda_x)) = [11, 10, 9, \ldots, 1]$, where the higher rank indicates the higher mean of the MAP values. Similarly, we use $R^i(Avg(Z, \lambda_x))$ to denote the $R(Avg(Z, \lambda_x))$ calculated on the dataset $i$. Finally, we compute the element-wise mean rank across the four datasets:

\begin{equation}\label{eq:avg_r_lambda_x}
    AvgR(Z,\lambda_{x})) = \frac{1}{n}\sum_{i=1}^{n}{R^i(Avg(Z,\lambda_{x}))},
\end{equation}
where $n = 4$ corresponding to the number of datasets. Using the above equation, we find the best value for $\lambda_{x}$ that is the $a \in Z$ generating the highest rank.

Finding the best value for $\lambda_d$ is the same as the above procedure, except that we fix $a$ to be the identified best value for $\lambda_x$.
Thus, Eq.~\ref{eq:avg_lambda_x} is modified as:
% \begin{equation}\label{eq:avg_lambda_d}
$Avg(b, \lambda_{d}) = {\textrm {MAP}} (a, b)$.
% \end{equation}
Then, we obtain the $|Z|$-length vector of $Avg(b, \lambda_{d})$ for all possible values for $b \in Z$. This vector is denoted as $Avg(Z, \lambda_d)$. Also, $R^i(Avg(Z, \lambda_d))$ indicates the $R(Avg(Z, \lambda_d))$ calculated on the dataset $i$. Finally, we compute the element-wise mean rank across the four datasets using the Eq.~\ref{eq:avg_r_lambda_x} except that $\lambda_x$ is replaced with $\lambda_d$.
% \begin{equation*}
%     AvgR(Z,\lambda_{d})) = \frac{1}{n}\sum_{i=1}^{n}{R^i(Avg(Z,\lambda_{d}))},
% \end{equation*} 
By doing so, we find the best value for $\lambda_{d}$ by choosing the $b \in Z$ generating the highest rank.
Fig.~\ref{fig:eval_lamb_XP}(a) - (b) show the average ranks of values in $Z$ for $\lambda_{x}$ and $\lambda_{d}$, respectively, across four datasets. As we see, $\lambda_{x}$ = $1.0$ produces the highest rank, whereas $\lambda_{d}$ = $0.7$ is the highest rank with $\lambda_{x}$ = $1.0$. The best ones are denoted in red color. 
% Finally, we choose these ones for $\lambda_{x}$ and $\lambda_{d}$ in \EF.

% Wiser
% nTFIDF

\begin{figure}[!h]
    \begin{minipage}[b]{0.45\linewidth}
        \centering
        \includegraphics[trim=0cm 0cm 0cm 0cm, width=105pt]{figures/best_x.pdf}
        \subcaption{}
    \end{minipage}
    \quad
    \begin{minipage}[b]{0.45\linewidth}\vspace{0pt}
        \centering
        \includegraphics[trim=0cm 0cm 0cm 0cm, clip, width=105pt]{figures/best_p.pdf}
        \subcaption{}
    \end{minipage}  
    \caption{Finding the best values for $\lambda_{x}$ and $\lambda_{d}$.}
    \label{fig:eval_lamb_XP}
\vspace{-10pt}
\end{figure}

\subsection{Evaluation of \EF}\label{sec:eval_ef}
We now evaluate \EF using the best values for $\lambda_{x}$ and $\lambda_{d}$. To measure its relative effectiveness, we also compare it with $n$VSM as well as two GMs: \textit{ADT}~\citep{Gollapalli:2013} and \textit{Reputation Model} (simply \textit{RepModel})~\cite{Daniel:2015}. Further, we compare \hits (Eq.~\ref{eq:hits_topic2}) with CO-HITS (Eq.~\ref{eq:hits_topic}) to validate the stronger capability of \hits's variation approach over CO-HITS. Finally, we show that \EF works well regardless of \textit{topic coverage}.

\begin{figure*}[!t]
\begin{center}
    \begin{tabular}{llll}
      \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/FLExR.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/FIR.pdf} & \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/FSW.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=39mm,height=40mm]{figures/FCL.pdf}
    \end{tabular}
    \caption{Comparison on the average precision (AP) values: x-axis shows n of P@n and y-axis shows AP values.}
    \label{tab:eval_APF}
\end{center}
\end{figure*}

\captionsetup[table]{labelfont=bf, skip=0pt}
\begin{table*}[!t]
    \caption{MAP and the the improvement ratio of \EF.}
    \begin{center}
        \scalebox{0.9}{
            \setlength{\tabcolsep}{9pt}
            \begin{tabular}{l r l r l r l r l r l}
            \hline
            & LExR & & IR & &  SW & & CL & & Avg. \\
            \hline
            $n$VSM & 0.666 & (12.1\%) & 0.222 & (15.3\%) & 0.106 & (7.6\%) & 0.106 & (4.7\%) & 0.275 & (11.6\%) \\            
            ADT & 0.574 & (30.1\%) & 0.186 & (37.6\%) & 0.077 & (48.1\%) & 0.106 & (4.7\%) & 0.236 & (30.1\%) \\
            RepModel & 0.260 & (187.3\%) & 0.144 & (77.8\%) & 0.061 & (86.9\%) & 0.070 & (58.6\%) & 0.134 & (129.1\%) \\
            CO-HITS & 0.611 & (22.3\%) & 0.228 & (12.3\%) & 0.104 & (9.6\%) & 0.088 & (26.1\%) & 0.258 & (19.0\%) \\
            % \EF* & 0.738 & (1.22\%) & 0.252 & (\textbf{1.59\%}) & \textbf{0.117} & (-2.56\%) & 0.108 & (2.78\%) & 0.304 & (0.99\%)  \\
            \EF & \textbf{0.747} & & \textbf{0.256} & & \textbf{0.114} & & \textbf{0.111} &  & \textbf{0.307} & \\        
            \hline
            \end{tabular}
        }
    \end{center}
    \label{tab:eval_MAPF}
% \vspace{-10pt}
\end{table*}

ADT uses an indirect and weighted tripartite (expert-document-topic) graph, where each triplet contains experts, documents and topics. 
Experts are connected to their documents, and also documents are connected to the topics based on their occurrences. The weight of an edge between an expert $x$ and a document $d$ ($w_{xd}$) corresponds to $p(x|d)$ in Eq.~\ref{eq:pw_2}. The weight of an edge between $d$ and a topic $t$ ($w_{dt}$) is modelled as $p(t|d)$ in Eq.~\ref{eq:pw_2}. Recall that we fixed $p(x|d)$ as 1 in Section~\ref{sec:eval_frame}.
As \EF models $p(t|d)$ as $n$TFIDF, we also model $w_{dt}$ as $n$TFIDF in ADT for the fair comparison.
% An example of $G$ is shown in Fig. \ref{fig:adt}, where we see two experts \{$x_1, x_2$\}, three documents \{$d_1, d_2, d_3$\}, and two topics \{$t_1, t_2$\}. 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=40mm,scale=1]{figures/adt.pdf}
%     \caption{An example graph in ADT.}
%     \label{fig:adt}
% \end{figure}
ADT ranks $x$ given a topic $t$ based on the  score function $s(x,t)$ (the higher the more important):
\begin{equation} \label{eq:adt_xt_1}
    s(x, t) = \sum_{d\in \mc{D}_{x}}{w_{xd} \cdot pweight(d,t)},
\end{equation}
where 
% $w_{xd}$ is 1 as stated above, and 
% $pweight(d,t)$ is defined as:
% \begin{equation} \label{eq:adt_dt}
    $pweight(d,t)$ = $\sum_{p \in P(d, t)}{\prod_{i}{w(e_i)}}$
% \end{equation}
where $p$ is a path between $d$ and $t$ comprising of edges such that $p = e_1e_2 \ldots e_n$; $P(d, t)$ is the set of all possible paths between $d$ and $t$; and $w(e_i)$ is the weight of the $i$-th edge in $p$. 
% We set the max length of $p$ to be 4 to reduce the exponential growth of the number of paths in $P(d,t)$.
% is a set of documents of expert $x$ and $w(x, d)$ is the weight of the edge in $p \in P(x, d)$. According to our (1) configuration, $|p(x, d)|\text{-length} = 1$ and $w(x, d) = 1$, thus, Eq. \ref{eq:adt_xt_1} can be written as:
% \begin{equation} \label{eq:adt_xt_2}
%     w(x, t) = \sum_{d\in \mc{D}_{x}}{w(d|t)}
% \end{equation}
% Let's define $P(x, d)$ and $P(d, t)$ are sets of all possible paths between $x$ and $d$ nodes and between $d$ and $t$ nodes respectively. The evaluation configuration for this approach includes: (1) with each given $t$ nodes, $G$ contains at most four $t'$ nodes, which are selected uniformly in the reference to $d$ nodes connected with $t$ node. This helps avoid the exponential growth in number of nodes  in $G$ causing the long computational time. (2) Accordingly, we fix $W_{ED} = 1$ and assign $n$VSM for $W_{DT}$, where $W_{ED}$ is weights of all edges between $x$ and $d$ nodes and $W_{DT}$ is weights of all edges between $d$ and $t$ nodes. (3) We also fix $\max{(|p(d, t)|\text{-length})} = 3$ where $p(d, t) \in P(d, t)$ and $|p(d, t)|\text{-length}$ is number of edges in $p(d, t)$. The weight of document $d$ given topic $t$ is estimated as \cite{Gollapalli:2013}:
% \begin{equation} \label{eq:adt_dt}
%     w(d|t) = \sum_{p \in P(d, t)}{\prod_{i}{w(e_i)}}
% \end{equation}
% where $w(e_i)$ indicates the weight of the $i^{\text{th}}$ edge in $p \in P(d, t)$. 
% Intuitively, to measure the weight of $x_{1}$ given $t_{1}$ in Fig. \ref{fig:adt}, we first generate all possible paths between $t_1$ and each $d$ node - that includes:
% $
%     \\
%     p(d_1, t_1) = \{ \{t_1, d_1\}, \{t_1, d_2, t_2, d_1\} \}, \\
%     p(d_2, t_1) = \{ \{t_1, d_2\}, \{t_1, d_1, t_2, d_2\} \}, \\
%     p(d_3, t_1) =  \{ \{t1, d_3\} \} \\
% $
% Then, $w(d|t)$ of each document is calculated by Eq. \ref{eq:adt_dt} as $w(d_1|t_1) = 0.454$, $w(d_2|t_1) = 0.372$, $w(d_3|t_1) = 0.5$. Finally, $w(x_1, t_1)$ is estimated by Eq. \ref{eq:adt_xt_2} as $w(x_1, t_1) = 0.872$.
% We also include RepModel~\cite{Daniel:2015} in our comparison. 
RepModel~\cite{Daniel:2015} was originally designed to estimate the topic-sensitive reputation of an organisation in the context of scientific research projects. This model uses topic-sensitive CO-HITS given a topic, where an organisation is seen as an expert and a project is seen as a document in our work. Thus, using the CO-HITS notations in Eq.~\ref{eq:hits_topic}, RepModel models $A(x;t)^k$ as  $\sum_{w\in t} w_wA(x;w)^k$ and  $H(d;t)^k$ as $\sum_{w\in t} w_wH(d;w)^k$, where $w_w = \frac{1}{|t|}$. As $\lambda_{x}$ and $\lambda_d$, we use 0.85 as used in \cite{Daniel:2015}. In RepModel, the personalised weights $\alpha_{x;w}$ and $\alpha_{d;w}$ are defined as: $\alpha_{d;w}$ = $tf(d,w)$ denoting the term frequency of $w$ divided by $|d|$;
% , where we note that \cite{Daniel:2015} did not use the topic-sensitive personalised weight for documents, not considering $w$ in $\alpha_{d;w}$; 
and $\alpha_{x;w}$ = ${s(x,w)}$ if $w$ appears in $\mc{D}_x$, and 0, otherwise. $s(x,w)$ is defined as $1 - \frac{\max_s - weight(x,w)}{\max_s - \min_s }$, where $\max_s$ and $\min_s$ are the max and min values of $weight(x,w)$ for all experts, and $weight(x,w)$ is the weight of $x$ on $w$ calculated by the number of documents in $\mc{D}_x$ where $w$ appears. We also set $k$=5 as done for \hits.

For the fair comparison between \hits and CO-HITS, as \hits, personalised weights $\alpha_{x;t}$ and $\alpha_{d;t}$ in CO-HITS in Eq.~\ref{eq:hits_topic} are set as $\mb{TX}_{i(t),i(x)}$ and $\mb{TD}_{i(t),i(d)}$, respectively. Following the same experiment in Section \ref{sec:lamb_eval}, we found that the best values for $\lambda_{x}$ and $\lambda_{d}$ are chosen as 1.0 and 1.0, respectively, for CO-HITS. 
% This means that CO-HITS shows the best performance without the personalised weights, exploiting only the authority and hub score propagation on the \ecg. 
We also fix $k$ as 5 in Eq.~\ref{eq:hits_topic} as \EF. In our comparison below, CO-HITS indicates an alternative \EF form incorporating $n$VSM into CO-HITS.


\begin{figure*}[!t]
\begin{center}
    \begin{tabular}{llll}
      \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=40mm,height=40mm]{figures/SLExR.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=40mm,height=40mm]{figures/SIR.pdf} & \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=40mm,height=40mm]{figures/SSW.pdf} &  \includegraphics[trim=1.8cm 0cm 0cm 0cm,width=40mm,height=40mm]{figures/SCL.pdf}
    \end{tabular}
    \caption{MAP values of $n$VSM and \EF: the x-axis shows topic coverage values, and the y-axis shows the MAP values (topic coverage of a topic $t$ means the number of known experts associated with $t$).}
    \label{fig:eval_ap_expert}
\end{center}
% \vspace{-10pt}
\end{figure*}

Fig. \ref{tab:eval_APF} shows the evaluation results based on the AP values with n (n=10,  15,  $\ldots$, 30) of P@n for all topics. First, when comparing \EF with ADT, although ADT is slightly better than \EF over two datasets IR and CL at n=10, \EF largely outperforms at all values for n of P@n, i.e. n=15, $\ldots$, 30, on all the datasets. It is also clear that \EF is substantially better than RepModel on all x-axis values.
% Also, ADT more steeply degrades its performance than \EF, as n of P@n increases. 
Second, \EF is consistently better than CO-HITS on LExR and SW, and very similar to each other on IR. On CL, CO-HITS is better than at n=10 and n=15, but similar at n=20, and worse than \EF at n=25 and n=30. Overall, these results also show that \hits can have a competitive potential for improving the performance over CO-HITS. Third, to determine the impact of incorporating $n$VSM into \hits in \EF, let us compare \EF with $n$VSM. As observed, \EF is clearly and consistently better than $n$VSM over LExR and SW, although they are similar on IR and $n$VSM looks better than \EF on CL. On average, we observe that our ensemble model \EF combining $n$VSM with \hits is observed to be more powerful than only $n$VSM. 
Table~\ref{tab:eval_MAPF} shows the evaluation results in MAP. The best one is denoted in boldface. As observed, \EF outperforms all the methods in 11.6\%, 30.1\%, 129.1\% and 19.0\% over $n$VSM, ADT, RepModel and CO-HITS, respectively, on average. Interestingly, $n$VSM is observed as the second better one. This also shows that our $n$VSM for expert finding is more competitive than the compared GMs.

Finally, it may be also worth analysing the distribution of the MAP values of a model across topics based on \textit{topic coverage} in each dataset. In our context, the topic coverage of a topic $t$ means the number of known experts having expertise $t$. This enlightens how the model particularly works better or worse at which topic coverage values. Intuitively, it may be harder to find experts for topics whose topic coverage is lower. For this analysis, we pay only attention to our two models $n$VSM and \EF. By comparing their distributions, we can identify which model is better than the other on what topic coverage values. 

The analysis results are seen in Fig.~\ref{fig:eval_ap_expert}. In each plot, each value on the x-axis shows a {topic coverage} value. Each value on the y-axis shows the MAP value of \textit{the set of topics with the same topic coverage}. For example, on LExR, the value 5 on the x-axis means that the topic coverage is 5. The corresponding y-axis value 0.85 indicates that the MAP value of the set of topics with the topic coverage 5 is 0.85. Each MAP value is also calculated using n=30 of P@n. Each black circle represents that both of $n$VSM and \EF have the same MAP value. We can observe the following: (1) On LExR, \EF dominantly outperforms or is equal to $n$VSM over all the topic coverage values except the 4 cases (i.e. 13, 15, 18, and 19); (2) On IR, \EF also shows its improvement over $n$VSM over most of the topic coverage values, while one MAP value is the same on the topic coverage 26; (3) On SW, we observe that \EF prevailingly outperforms $n$VSM across most of the topic values as \EF's distribution is predominantluy higher than $n$VSM's distribution; (4) On CL, although $n$VSM is better than \EF on the topic coverage values 10 and 30, \EF is observed notably better than $n$VSM over the other topic coverage values; and (5) there seems no clear clue that \EF performs particularly better on which range of topic coverage. For example, on LExR, \EF seems to perform better in smaller topic coverage values, as the MAP values from 0 to 5 are clearly higher than those from 6 to 15 on the axis. But this pattern is not consistent with the datasets on SW and CL, where \EF performs better on larger topic coverage values. In conclusion, the above observations may indicate that overall \EF outperforms $n$VSM regardless of topic coverage, showing the validity of the design paradigm of \EF, that is, incorporating $n$VSM into \hits can have powerful capability for expert finding.

% We observe the following: (1) While ADT outperforms others with P@10, \EF improves consistently over all the four datasets from P@15 to P@30; (2) \EF outperforms \hits on all the four datasets, this shows incorporating $n$VSM into CO-HITS improves the performance of CO-HITS.

% We now evaluate \EF in MAP with n=30 with P@n.

% \yb{Add the explanation about \EF*}


% We now analyse the evaluation results of the compared methods based on the average of the P@n values (AP) for all topics in each dataset and MAP. Fig. \ref{tab:eval_APC} illustrates the AP values with n (n=10, 15, $\ldots$, 30) of P@n for all topics. We observe the following: (1) Overall, the VSM approach (TFIDF and $n$VSM) largely outperforms both DLM-0.5 and DML-0.6. This indicates the VSM approach can be more effectively used for identifying topic-sensitive experts than DLM approaches; (2) $n$VSM is clearly better than TFIDF from P@10 to P@30 consistently over the all the four datasets. Also, $n$VSM highly outperforms DLM-0.5 and DLM-0.6 over all the AP values on all the four datasets. This shows that a good potential of $n$VSM for expert finding.

% We now evaluate $n$VSM in MAP with n=30 of P@n. Table \ref{tab:eval_MAPC} shows the MAP values of the four methods and the relative improvement ratio of $n$VSM over the other three methods. The best one in each dataset is denoted in boldface. We observe that $n$VSM largely outperforms DLM-0.5 in 103.7\%; DLM-0.6 in 133.1\%; and TFIDF in 21.7\% on average across the four datasets. Although TFIDF is better than $n$VSM on CL, it is worse than $n$VSM over the other 3 datasets. In conclusion, we can claim that $n$VSM performs very well and achieves much better performance than DLM and TFIDF-based VSM approaches. This is a good evidence that our $n$VSM approach can be effectively used for expert finding.

\subsection{Discussions and Future Work}\label{sec:discussion}

% Ratio Expert Finder - DLM (2) - TFIDF

% Below is the ratio improvements of \EF with DLM and TFIDF.
% \captionsetup[table]{labelfont=bf, skip=0pt}
% \begin{table*}[!t]
%     \caption{MAP and the the improvement ratio of \EF.}
%     \begin{center}
%         \scalebox{0.9}{
%             \setlength{\tabcolsep}{9pt}
%             \begin{tabular}{l r l r l r l r l r l}
%             \hline
%             & LExR & & IR & &  SW & & CL & & Avg. \\
%             \hline
%             DLM-0.5 & 0.200 & (273.5\%) & 0.208 & (23.1\%) & 0.070 & (62.9\%) & 0.063 & (76.2\%) & 0.135 & (127.4\%) \\
%             DLM-0.6 & 0.159 & (369.8\%) & 0.185 & (38.4\%) & 0.068 & (67.7\%) & 0.058 & (91.4\%)  & 0.118 & (160.2\%) \\
%             TFIDF & 0.493 & (51.5\%) & 0.206 & (24.3\%) & 0.087 & (31.0\%) & \textbf{0.120} & (-7.5\%) & 0.226 & (35.85\%) \\
%             \EF & \textbf{0.747} & & \textbf{0.256} & & \textbf{0.114} & & 0.111 &  & \textbf{0.307} & \\        
%             \hline
%             \end{tabular}
%         }
%     \end{center}
%     \label{tab:eval_MAPF}
% \end{table*}

Using the four datasets from academic domains, we evaluated \EF and its two key components  $n$VSM and \hits, and compared the results with  other expert finding models: TF-IDF based VSM (denoted as TFIDF), DLM-0.5~\cite{Balog:2009} and DLM-0.6~\cite{Wang:2015}, WISER~\cite{WISER:2019}, ADT~\cite{Gollapalli:2013} and RepModel~\citep{Daniel:2015}. 

We showed the capability of $n$VSM using different AP values (n=10, 15, $\ldots$, 30) and MAP, in comparison with TFIDF, DLM-0.5 and DLM-0.6. 
% over a typical DLM approach~\cite{Balog:2009, Wang:2015} with two configurations denoted as DLM-0.5 and DLM-0.6, a recent WISER, and a TFIDF-based VSM approach denoted as TFIDF. 
On average, the improvement ratio of $n$VSM over them was turned out as from 21.7\% to 133.1\% in MAP. We also presented the empirical method for finding the best values of the two parameters used in \EF, $\lambda_x$ and $\lambda_d$, based on the ranking of the MAP values. Moreover, we showed how much \EF performs better than all the compared methods in Table~\ref{tab:eval_MAPC} and Table~\ref{tab:eval_MAPF} in MAP. That is, we showed that \EF improves DLM-0.5 and DLM-0.6 in 127.5\% and 160.2\%, respectively; TFIDF in 35.9\%; WISER in 71.5\%; ADT in 31\%; $n$VSM in 11.6\%; RepModel in 129.1\%; and CO-HITS in 19.0\%. 
Further, we showed that \EF incorporating $n$VSM into \hits indeed improves only $n$VSM. It means that exploiting network propagation effects on \ecg using \hits with the outcome of $n$VSM can contribute to better estimating topic-sensitive weights of experts. Also, by comparing \EF with a model combining $n$VSM with CO-HITS, we proved that \hits can be an effective approach for improving CO-HITS for expert finding.
Finally, we analysed that \EF works well regardless of topic coverage values. Our all evaluation results reinforce our motivation of designing \EF that the proposed ensemble model \EF for expert finding is effective and competitive for expert finding. 


% Our experiments are comprehensive as we analysed the effectiveness of \EF, in comparison with representative approaches of VSM, DLM and GM on the four different datasets, as well as we provided in-depth analysis of \EF showing the prominent capability of the two key components ($n$VSM and \hits) incorporated in \EF. Note that \EF is a hybrid approach equipped with the state-of-the-art $N$-gram IDF method~\cite{nidf:2017} and a novel idea based on the CO-HITS equation.

As future work, it could be worth to try to find a way for improving precision for expert finding. As we have observed in Table~\ref{tab:eval_MAPF}, the average MAP value of \EF is 0.307 across the four datasets. In the literature, we can also observe the similar MAP results. For example, WISER~\cite{WISER:2019} reported that its best MAP values are 0.214 and 0.363 on the two datasets, BMExpert~\cite{Wang:2015} also showed 0.06 as the best MAP value of the DLM~\cite{Balog:2009} on the single dataset, and ADT~\cite{Gollapalli:2013} also showed its best MAP values are 0.0943 and 0.1986 on the two datasets. 
% Also, \EF's MAP values are very different depending on the datasets. On LExR, the MAP value is relatively high (i.e. 0.747), while on CL it is much low (i.e. 0.111).
As another future work, we plan to accommodate a general expertise knowledge source as ~\cite{WISER:2019}, e.g. Wikipedia, into \EF to see its potential for enhancing
\EF's capability. Another interesting future work is that we could examine graph embedding techniques for expert finding. One idea would be that we extend \ecg by constructing an expert-document-topic graph based on their semantic relationships. Then we can train a machine to transform nodes, edges and their features into a vector space while maximally preserving their relationship information. Once we would be successfully able to map such a graph to a vector space,  we could estimate the importance of experts given documents or topics by measuring their similarity (or relevance) between experts and documents or between experts and topics in terms of their corresponding vector values. 


% Another potential future work may be is to construct an expert knowledge graph reflecting the relationships between experts, documents and topics, and their inter-relevance could be answered using semantic queries over the graph.


==> Expertise Retrieval_TKDE/intro.tex <==

\section{Introduction}\label{sec:intro}
{Finding experts in a particular domain} is key to accelerate rapid formation of teams to respond to new  opportunities, as well as undertake and address new frontiers in research innovations. Further, accurately identified experts can significantly contribute to enhancing the research capabilities of an organisation leading to higher quality research outcomes. In general, an \textit{expert} is defined as a person who has sufficient knowledge and skills in a given field~\citep{husain2019expert}. Such knowledge and skills are called \textit{expertise}. While digitally available data  (e.g. scientific publications) describing expertise of experts is rapidly growing, manually collating such information to find experts seems impractical and expensive. Thus, often in a large research organisation with diverse disciplines, finding experts in a field that one does not know or has limited knowledge is particularly very challenging.
%that it is increasingly hard for people to seek experts. 
%Second, in a large research organisation with diverse disciplines, it is particularly challenging to find experts in a field that one does not know or has \amir{"a" is not needed. Should be "limited knowledge"}a limited knowledge about it. Thus, finding experts requires comprehensive information about people who can solve the questions of expert seekers. 
% However, manually collecting such information seems impractical when considering the challenges described above. 
%and exploiting their expertise have a powerful impact on improving  and products in a scientific or technology domain. 
%Also, accurately identified experts in such a domain are a key asset that accelerates \amir{the} rapid formation of teams to respond to new  opportunities.
%However, there still remains \amir{remain} some challenges. 
% First, the breadth and depth of knowledge areas grow rapidly in a scientific and innovation domain. 

Information retrieval techniques have been widely used to aid retrieval task for finding experts from digitally available expertise data (we collectively term these as \textit{documents} in this paper)
%\amir{how about changing "expertise evidences" to "resources" } 
 such as scientific publications~\citep{Stankovic2010LookingFE}. 
%In this paper, we collectively see these evidences \textit{documents} to simplify our presentation. 
%\amir{There are so many use of the work "expert" in this text. Exactly 9 times in one paragraph. Makes it difficult to read. I suggest remove some of them if possible.}
Based on the literature~\cite{gonccalves2019automated}, there are two specific tasks for expert retrieval: (1) \textit{expert finding} - identifying experts given a topic from available documents and rank them based on their expertise level, and (2) \textit{expert profiling} - identifying the areas of expertise given an expert.
In this paper we focus on the first task (i.e. {expert finding}) and propose an ensemble model for it from unstructured documents. We use the term \textit{topic} to represent a field of  expertise.
% , and a topic is represented as a single term or a phrase.

% An earlier study shows~\citep{Balog:07} that these two tasks have a common mathematical ground as both are commonly interested in building an \textit{expert-topic matrix} and sorting the values along one of the dimensions. However, expert finding focuses more on examining techniques to find experts from documents associated with a topic, while expert profiling concentrates more on techniques to find topics from documents associated with a specific person. 

Most existing approaches for expert finding are based on \textit{vector space models} (VSM), \textit{document language models} (DLM), or \textit{graph-based models} (GM).
In VSM, expert finding is often solved by modeling the weights of topics, associated with the documents produced by experts, using Term Frequency-Inverse Document Frequency (TFIDF) or its variation~\citep{chuang2014combining,alhabashneh2017fuzzy}. 
% VSM~\citep{Salton:86} models the documents and terms into a vector space, where a document is represented as a vector and its elements are terms appearing in the given document collection. 
In DLM, expert finding is achieved by estimating the probability that a topic would be observed in the documents of an expert~\citep{Balog:2009, Wang:2015,WISER:2019}. 
In GM, a graph is used to represent associations among experts, documents and/or topics. The  strengths of the associations are inferred to estimate the expertise degree of an expert given a topic using various graph analytics such as expert-document-term association paths~\citep{Gollapalli:2013}, Hyper-Induced Topic Search (HITS)~\citep{Campbell:2003,Yeniterzi:2014}, or social network based link analysis methods~\cite{faisal2019expert,bok2019expert,Sziklai:2018}.

% However, their experiments considered very small networks (less than 15 people) and failed
% to explain the meaning of hub and authority in HITS in the context of
% expert finding

Although various models in these approaches aforementioned have been proposed, integrating VSM and GM for expert finding has been little studied in the literature. In this work, we propose an ensemble model for expert finding, \textit{\EF}\footnote{ExpFinder's source code is publicly available on\\ \url{https://github.com/Yongbinkang/ExpFinder}}, that integrates a novel $N$-gram VSM, denoted as $n$VSM, with a GM using an \textit{expert collaboration graph (ECG)}. We develop $n$VSM for estimating the expertise degree (or \textit{weight}) of an expert given a topic by leveraging the recent Inverse Document Frequency (IDF) weighting~\citep{nidf:2017} for $N$-gram words (simply $N$-grams) composed of two or more terms (for N$>$1). This method demonstrated a higher robustness and effectiveness in measuring the IDF weights of $N$-grams.
We also build an \ecg in the form of an expert-document bipartite graph to represent the associations between experts and documents based on the co-authorship information.
% \amir{Just a note for future investigation: Is CO-AUTHORSHIP network complete and valid? These networks tend to be highly in accurate given the poor disambiguation method for author names. This also might be something to mentioning as "threats to validity"}
% \prem {perhaps include Amir's concern as part of assumption/limitation of the work or as future work}
To estimate the weight of an expert given a topic on the \ecg, we propose the GM, \hits, that is formed by applying two variation schemes to the generalised CO-HITS~\citep{Hongbo:2009} algorithm. 
%\EF is an ensemble model as, given a topic $t$, it incorporates the estimated weights of experts in the $N$-gram VSM, into \hits, to further reinforce the estimation of the degrees of relevant experts for $t$. 

% Although some HITS algorithms were previously used for expert finding, \EF differs in that (1) \hits is a \textit{topic-sensitive} HITS like algorithm, where the weights of experts are estimated given a topic, but the prior works used topic-independent HITS algorithms~\citep{Campbell:2003,Yeniterzi:2014}; 
% (2) \hits works on an \ecg, while \citep{Campbell:2003,Yeniterzi:2014} applied HITS on an expert-expert graph; and (3) \hits is a variation of CO-HITS~\citep{Hongbo:2009}. 
% In CO-HITS, an authority score (i.e. expert weight) is computed as the \textit{sum} of the hub scores (document weights) that point to that authority (expert). Also, a hub score is the \textit{sum} of the authority scores that the hub (document) points to. These authority and hub scores are mutually updated one another repeatedly. However, \hits calculates an authority score by the \textit{average} of the hub scores that point to that authority. Also, a hub score is calculated by the \textit{average} of the authority scores that the hub points to. 
% % Also, \hits is topic-sensitive, meaning that the authority and hub scores are calculated for a given topic.
% In our evaluation, we show the outperformance of \hits over CO-HITS.

This paper makes three main contributions. First, to our best knowledge, \EF is the first attempt to introduce $n$VSM for expert finding. 
% To estimate the weights of topics, where a topic consists of multiple-terms, we propose a TFIDF metric for $N$-grams, named {$n$TFIDF}. To generate $n$TFIDF, we utilise the $N$-gram IDF method~\cite{nidf:2017}.
Second, we propose \EF an ensemble model that combines $n$VSM and the GM using \hits to create a stronger model for expert finding that achieves better performance than a single one. \EF incorporates the weights of experts estimated by $n$VSM into an \ecg and uses \hits on the \ecg to better estimate the weights of experts for a given topic. Third, we conduct comprehensive empirical evaluations to measure the effectiveness of \EF using four different datasets (LExR~\cite{Vitor:2016} and three DBLP datasets~\cite{bordea2013benchmarking}) in academic domains and compare the results with six different expert finding models: the  TFIDF-based VSM, two DLMs~\citep{Balog:2009,WISER:2019} and three GMs~\citep{Gollapalli:2013,Daniel:2015,Hongbo:2009}. 
% Prior works, leveraging HITS, for expert finding  used a very small email communication dataset (around 15 expert)~\citep{Campbell:2003} and a single Web blog dataset, thus hard to to see the impact of HITS for expert finding. 
% We also show the effectiveness of nVSM, in comparison with the traditional TF-IDF based VSM approach. 
%Further, we present in-depth analysis of \EF, as well as show a substantial outperformance of \EF, in comparison with 

% To address the above issues, we have designed and developed \EF. \EF is a novel retrieval method for identifying expertise characterised by their relevant expertise concepts by incorporating semantic analysis of text-based evidence (e.g. scientific publications or patents) of the experts as well as an expert collaboration network in a given domain. In our preliminary evaluation, it turns out that \EF outperforms several state-of-the-art approaches for expertise retrieval.

This rest of the paper is organised as follows. Section~\ref{sec:related_work} provides related works in expert finding. Section~\ref{sec:overview} presents an overview of \EF and Section~\ref{sec:design} discusses in-depth steps for building \EF. 
Section~\ref{sec:eval} presents thorough empirical evaluations of \EF, followed by conclusion in Section~\ref{sec:conclusion}.


==> Expertise Retrieval_TKDE/overview.tex <==

\section{Introduction to ExpFinder}\label{sec:overview}
In this section, we present the overview of \EF, and  the basic notations that we will use in the paper. 

\subsection{Overview of ExpFinder}
% The objective of \EF is two-fold. {First}, \EF aims to identify right expertise of a given expert, where such  expertise  is represented by a set of topics ranked according to their relevance to the expert (i.e. expert profiling). As such topics, we choose to use
% keyphrases\footnote{In our work, expertise topics are modelled using keyphrases so that we use these terms interchangeably.} which are extracted from the expert's text-based evidence such as research publications or patent descriptions. For the sake of simple presentation and illustration, as such an evidence, we focus on \textit{publications} of experts in this paper.
% A keyphrase is defined as a representative and characteristic phrase consisting of one or more terms extracted from the given publications. Keyphrases have been widely used to represent expertise topics~\citep{Rodrigo:2019,Eirini:20}
% {Second}, \EF focuses on finding right experts given a set of expertise topics in the target domain (i.e. expert finding).
\EF aims to identify ranked experts according to their expertise degree given a topic. In this paper, we assume that a topic is represented as a \textit{noun phrase} which is extracted from documents (e.g. scientific publications) of experts in a given domain. The reason is that domain-specific concepts are often described by noun phrases that represent the key information within a given corpus~\cite{Kang:2014}. 
%For the sake of presentation, we collectively call such evidence \textit{documents}.
A noun phrase  means  a  single-word noun or a group of words that function together as a  noun.  
% A keyphrase is defined as a representative phrase consisting of one or more terms extracted from the given documents. Keyphrases have been widely used to represent expertise topics~\citep{Rodrigo:2019,Eirini:20}
% {Second}, \EF focuses on finding right experts given a set of expertise topics in the target domain (i.e. expert finding).

The key of \EF is the utilisation of \textit{two knowledge facets} in a unified manner. The one is the estimation of the weights of experts given a topic by utilising information in the proposed $n$VSM. 
% The $N$-gram VSM uses vectors to represent documents. The elements of a vector consist of topics (i.e. keyphrases) appearing in the given documents. This forms a document-topic matrix. 
% The rows are defined as documents in the vector space while the columns of the matrix are defined as the topics used to describe the documents in the vector space.
% An entry of the matrix reflects the weight of a topic assigned to a document. The weight is estimated using $n$TFIDF in our approach. 
% Using this scheme, we  generate topic-expert and topic-document matrices, where each entry indicates the weight of each expert and document given a topic, respectively. 
The second facet is \hits %\amir{what is ECG? It is not described or introduced before!}
that performs on an expert collaboration graph (\ecg), where the expert collaboration is measured by the joint production of experts (e.g. co-authored documents). We incorporate the result of $n$VSM into the \ecg, and reinforce the weights of experts given a topic using \hits.
The following presents the key steps in \EF (see also Fig.~\ref{fig:system_overview}):
% In this paper, we integrate these two knowledge facets into a unified manner for expertise retrieval\footnote{In the rest of this paper, expertise retrieval refers to expert profiling and expert finding.}


% degree of probability that a given expertise topic is relevant to an expert using a language model. A language model is based on the scheme of how frequently keyphrases appear in the given publications~\citep{Rodrigo:2019}. The second knowledge facet is an \textit{expert collaboration graph} (\ecg), where the collaboration is measured based on the joint production of experts (e.g. co-authored publications). In this paper, we integrate these two knowledge facets into a unified manner for expertise retrieval\footnote{In the rest of this paper, expertise retrieval refers to expert profiling and expert finding.}


\begin{figure}[!t]
\centering
\includegraphics[trim=0cm 0cm 0cm 0cm, clip,width=240pt]{figures/system_overview.pdf}
\caption{The overview of \EF.}\label{fig:system_overview}
\vspace{-10pt}
\end{figure}

{\textbf{Step 1: Extract topics}}: Given experts and their documents (also called \textit{corpus}) in a given domain, we extract noun phrases as topics. 
% For this, we apply a part-of-speech (POS) tagger to the corpus data. 
% Thus, the output of this step is the set of noun phrases extracted from the corpus. 
    % : (1) adjective nouns: adjective(s) followed by a sequence of nouns; (2) multiple noun: a sequence of nouns; and (3) single noun. 
    
    % For this purpose, we use the state-of-the-art keyphrase algorithm, YAKE!\cite{YAKE:2020}~\footnote{\url{https://github.com/LIAAD/yake}}
    
\textbf{Step 2: Estimate the weights of experts and documents given topics}: Given a topic, we estimate the weights of experts and documents based on the proposed \textit{$n$TFIDF} method in $n$VSM. In this paper, we also call such weights  \textit{topic-sensitive weights} as these weights are sensitive to the given topic. 
% $n$TFIDF estimates the weight of a topic given a document using the IDF method~\citep{nidf:2017} for the $N$-grams of the topic.
% each expertise topic based on a language model, taking into account its frequency and its inverse document frequency over all the publications of the expert. 
    % Note that YAKE! focuses only on extracting keyphrases from a single document, not considering their importance over all the publication corpus. 
% Note that some keyphrase extraction algorithms (e.g.YAKE!~\citep{YAKE:2020}) focus only on extracting keyphrases from a single document, not considering their importance over the given corpus. Thus, in order to accommodate various keyphrase methods into \EF and to make it generalisable, we propose a method for estimating the weights of the keyphrases for each publication and each expert. 
Given a topic, the key of $n$TFIDF lies in a combination of the frequency of the topic with the IDF method of $N$-grams over the corpus~\citep{nidf:2017}. The  output of this step includes a topic-expert matrix and a topic-document matrix, where an entry reflects the weight of an expert and a document given a topic, respectively.
    
\textbf{Step 3: Construct an ECG}: We construct an \ecg to represent associations between experts and their jointly-published documents. This graph is modelled by a \textit{directed, weighted bipartite graph} that has two kinds of nodes, one representing experts and the other representing documents. 
% Each expert is not connected to any other experts, and the same is with the documents. 
A directed edge points from a document $d$ to an expert $x$, if $x$ has published $d$. 
% Given an edge between an expert and a document, the weight of each edge is estimated by considering the importance (or weight) of the expert on the document. 
% Figure~\ref{fig:system_overview} shows  an example \ecg, where there are three experts  $\{x_1, x_2, x_3\}$ and three documents $\{d_1, d_2, d_3\}$. We see that $x_1$ has $\{d_1,d_2\}$, $x_2$ has  $\{d_1, d_2, d_3\}$, and $x_3$ has $\{d_3\}$; and $d_1$ and $d_2$ were published by $\{x_1, x_2\}$, and  $d_3$ by $\{x_2, x_3\}$.

\textbf{Step 4: Reinforce expert weights using \hits}:
As presented above, to rank experts, \EF integrates the two knowledge facets: (1) $n$VSM to estimate the weights of the experts and documents given a topic ({\textbf{Step 2}}); and (2) \hits incorporating such weights into an \ecg ({\textbf{Step 3}}) to further reinforce the weights of experts. 
% The \ecg will be used to estimate the relative importance of experts and publications using  the \hits algorithm. 
% This algorithm is based on the duality relationships embedded in mutual reinforcement between \textit{hubs}  and \textit{authorities} on \ecg. Hubs and authorities are referred to as documents and experts, respectively, in this paper.
% Specifically, we formulate the expert finding problem as a topic-sensitive HITS problem, where we estimate the authority scores of experts given an expertise topic.
The outcome of this step is the reinforced topic-expert matrix showing the weights of experts. Finally, we rank the experts for each topic from the matrix.
    
    % . We estimate the weights of expertise topics on each expert by designing an unifying function that integrates the following two information facets: 
    % \begin{itemize}
    % \item \textit{Estimation of the weight of an expertise topic for an expert using a language model}: A language model has been often used in expertise retrieval~\citep{Balog:2009, Wang:2015}, where the idea is to estimate the probability of a person being expert on an expertise topic or the probability of an expertise topic describing expertise for a given expert using a language model. More specifically, a language model can be used to estimate the probability of a term given a publication so that it can be used to answer the question like ‘what is the probability of seeing this term given this document?'. In our language model, in order to estimate the probability of a person being expert on an expertise topic, we calculate the following factors being integrated together: (1) the importance of an expertise topic to a document, (2) the importance of a publication, (3) a decaying factor of an expertise topic over time, and (4) the importance of an expert for a publication.

    % \item \textit{Estimation of the authority score of an expert for a publication with respect to expertise topics within the context of the ECG graph}: This authority score is based on the intuition that a publication is considered to be important if the experts contributing to it are also considered to be important within the expert collaboration environment drawn from ECG. Also, in turn, an expert is considered to be important if its publications are considered to be importance. This mutual, recursive intuition is modelled by using HITS (Hyperlink-Induced Topic Search)~\citep{Kleinberg:1999}. We define a variant HITS algorithm on the expert collaboration network to infer the authority  score of an expert for the publications of the expert with respect to expertise topics, satisfying the above intuition traversing ECG.
    % \end{itemize}

\subsection{Notations}\label{sec:notation}
We present the following basic notations in this paper.
\begin{itemize}
    \item Let $\mc{X}$ be the set of experts, and $|\mc{X}|$ be the number of experts in $\mc{X}$.
    \item Let $\mc{D}$ be the set of all documents published by $\mc{X}$. Let $\mc{D}_x$ be all documents published by $x \in \mc{X}$. Also, let $\mc{X}_{d}$ denotes the set of the experts that have a document $d \in \mc{D}$
    % \footnote{To simplify presentation, we sometimes omit the subscript of an element in a set, unless the subscript conveys an important meaning: e.g. $e$ and $d$ instead of $e_i$ and $d_j$, respectively.}.
    %\item Let $\mc{Y}$ be the set of the published years of $\mc{D}$.
    \item Let $\mc{T}$ be the set of topics extracted from $\mc{D}$. 
    % Let $\mc{T}_x$ be the set of topics of  $x \in \mc{X}$. \yb{do we use?}
    
    \item Let $\mb{TX}$ be a $|\mc{T}| \times |\mc{X}|$ topic-expert matrix where rows and columns are labeled with $\mc{T}$ and $\mc{X}$, respectively. The entry that lies in the $i$-th row and the $j$-th column of $\mb{TX}$ is denoted as $\mb{TX}_{i,j}$ that indicates the weight of $x_j \in \mc{X}$ on $t_i \in \mc{T}$. 
    % The weights are  represented by real numbers in [0,1]. 
    If a weight is higher, the more important the corresponding expert is on the given topic. 

    \item Let $\mb{DX}$ be a $|\mc{D}| \times |\mc{X}|$ document-expert matrix where rows and columns are labeled with $\mc{D}$ and $\mc{X}$, respectively. The entry of $\mb{DX}_{i,j}$ shows the weight of an expert $x_j \in \mc{X}$ on a document $d_i \in \mc{D}$ based on $x_j$'s contribution towards $d_i$.
    
    % \item Let $\mb{XT}$ be a $|\mc{X}| \times |\mc{T}|$ matrix where rows and columns are labeled with $\mc{X}$ and $\mc{T}$, respectively. The entry of the $i$-th row and the $j$-th column of $\mb{XT}$ is denoted as $\mb{XT}_{i,j}$ that represents the relative importance (or weight) of topic $t_j \in \mc{T}$ on expert $x_i \in \mc{X}$. This weight is represented as a real number in [0,1] and the sum of the weights of all experts on a topic $t_j$ is 1, i.e. $\sum_{x_k \in \mc{X}} \mb{XT}_{k,j}=1$. Also, the $i$-th row represents a $|\mc{T}|$-dimensional vector that shows the relative weight distribution terms in $\mc{T}$ on $x_i$. Regarding a weight, the higher, the more important $t_j$ is considered on $x_i$; or the better expertise $x_i$ has on $t_j$. 
    
    \item Let $\mb{TD}$ be a $|\mc{T}| \times |\mc{D}|$  topic-document  matrix where rows and columns are labeled with $\mc{T}$ and $\mc{D}$, respectively. $\mb{TD}_{i,j}$ represents the weight of document $d_j \in \mc{D}$ on $t_i \in \mc{T}$. 
    % Similarly, given an expert $x$, let $\mb{TD}_x$ be a $|\mc{T}_x| \times |\mc{D}_x|$ matrix where rows and columns are labeled with $\mc{T}_x$ and $\mc{D}_x$, respectively. \yb{do we use?}
    % The weights are represented by real numbers in [0,1].
   If a weight is higher, the more important the corresponding document is on the given topic. 
    
    % \item Let $\mb{TX}$ be a $|\mc{T}| \times |\mc{X}|$  topic-expert  matrix where rows and columns are labeled with $\mc{T}$ and $\mc{X}$, respectively. $\mb{TX}_{i,j}$ represents the relative weight  of expert $x_j \in \mc{X}$ on topic $t_i \in \mc{T}$ over $\mc{X}$.  
    % The weights are represented by real numbers in [0,1].
    % Regarding the weight, the higher, the more important an expert is on a given  topic\footnote{To simply the presentation, if a expert (or a topic) is given as $x$ (or $t$), instead of $x_j$ (or $t_i$) without a subscript, its entry in $\mb{TX}$ is denoted as $\mb{TX}_{t,x}$. This is also applied to $\mb{XD}$ and $\mb{DT}$.}.
    
    
    %and the sum of the weights of all publications on topic $t_j$ is 1, i.e. $\sum_{d_k \in \mc{D}} \mb{DT}(k,j)=1$. Also, $i$-th row represents a $|\mc{T}|$-dimensional vector that shows the relative weight distribution term in $\mc{T}$ on $d_i$. Regarding a weight, the higher, the more important $t_j$ is on $d_i$. 
    % \item Let $\mb{af}=[af_1, ..., af_{|\mc{D}|}]$ be a $|\mc{D}|$-dimensional vector (named \textit{age-dampening factor vector}), where the $i$-th value shows the age-dampening factor that penalises publication $d_i \in \mc{D}$ based on its published year. The older publications will have lower values in $\mb{af}$, normalized to real numbers between 0 (the oldest publication) and 1 (the latest publication) in $\mc{D}$.
    
    % \item To denote a column and row vector in a given matrix $\mb{M}$, we will use ${\mb{M}}$ with a subscript and mark `*'. For instance, the $i$-th row vector in $\mb{TX}$ is denoted as ${\mb{TX}}_{i,*}$, and the $j$-th column vector as ${\mb{TX}}_{*,j}$.
    
    % \item Let $\vec{\mb{dw}}=[dw_1, ..., dw_{|\mc{D}|}]$ be a $|\mc{D}|$-dimensional vector (named \textit{publication weight vector}), where the $i$-th value denotes a weight of publication $d_i$ in $\mc{D}$. The weight ranges from 0 to 1, interpreting that the higher, the more important.
    
    % \item Let $\vec{\mb{tw}}=[tw_1, ..., tw_{|\mc{T}|}]$ be a $|\mc{T}|$-dimensional vector (named \textit{domain-specific term weight vector}), where the $i$-th value denotes a domain-specific weight of term $t_i \in \mc{T}$. This weight is also normalised in [0,1], interpreting that the higher, the more important.
\end{itemize}




==> Expertise Retrieval_TKDE/related_work.tex <==
\section{Related Work}\label{sec:related_work}

In recent years, with the growing amount of digital expertise sources, expert finding has become an intensive research area in information retrieval community~\cite{gonccalves2019automated}.
We can mainly classify expert finding approaches into three categories: VSM, DLM and GM. 
% More recently, a mixture model combining these approaches also has gained popularity~\cite{kundu2019formulation}. 
% \yb{this reference is not for expert finding. need to find recent one} 

%Schunk:2010,riahi2012finding,chuang2014combining,alhabashneh2017fuzzy
In the VSM approach,
% \cite{Schunk:2010,riahi2012finding,chuang2014combining, alhabashneh2017fuzzy}, 
the common idea is to estimate relevance between a document and a topic using a weighting scheme in VSM (e.g. TFIDF or its variation). Then, finding experts can be done by assuming that an expert is seen as the collection of its published documents $\mc{D}_x$. That is, the weight of an expert $x$ given a topic $t$ is estimated by aggregating relevance scores between each document in $\mc{D}_x$ and $t$.
For example,  TFIDF  was used to find experts in community question answering websites in which the goal is to find users with relevant expertise to provide answers for given questions~\cite{riahi2012finding}. A variation of TFIDF was also applied for expert finding in an organization’s ERP system~\cite{Schunk:2010}. The work~\cite{chuang2014combining} also used TFIDF to identify experts given a topic using a topic extension method (finding interrelated terms of a given topic from the corpus), where TFIDF was used to estimate relevance between extended terms and each expert's documents. TFIDF was also used to estimate the weights of topics indicating the interests of an expert, and this information is used with fuzzy logics for expert finding~\cite{alhabashneh2017fuzzy}.

% Authors in \cite{alhabashneh2017fuzzy} created fuzzy relevance profiles using TFIDF analysis in their expert finding systems. They combined three profiles into a unified index reflecting the semantic weight of the query terms related to the task, user and document to select the most relevant documents and experts related to the query topic. 

% Authors in \cite{balog2008non} used TFIDF for identifying non-local aspects of document-expert associations for their expert finding model in enterprise settings. 

The aim of the DLM approach
% ~\cite{Balog:2009, Wang:2015, van2016unsupervised, Mangaravite:2016,WISER:2019} 
is to find experts whose documents are directly related to a given topic.
% The expert finding problem is mapped to multiple document features such as levels of associations between experts, documents and topics. 
In common, this approach estimates the relationships between a topic and an expert as the probability of generating the topic by the expert \cite{Balog:2009}, or between an expert and its publications~\cite{Mangaravite:2016}. BMExpert~\cite{Wang:2015} used the DLM~\cite{Balog:2009} for expert finding using three factors: relevance of documents to the topic, importance of documents, and associations between documents and experts. Similarly, the work \cite{van2016unsupervised} used a probabilistic DLM for expert finding by probabilistically generating a textual representation of an expert according to his documents and then ranking such documents according to a given topic. Recently, a probabilistic model, \textit{WISER}~\cite{WISER:2019}, estimated the importance of experts' documents given a topic using  BM25~\cite{BM25:2009}. Using this importance, such documents were ranked and these ranks were summed to represent the topic-sensitive weight of an expert.

% Authors in \cite{doval2019comparing} introduced $N$-gram based language model for word segmentation purpose. A major drawback of language model is the number of relationships between experts and topics are very limited and the method of combining them are mostly heuristic and not clearly justified \cite{Rodrigo:2019}. 
% \yb{any papers comparing the performance of language model-based approaches vs some other approaches? That'll be great if we can have such papers pinpointing the limitation vs performance....}

%\yb{include references 11-13, see intro}
In the GM approach,
% ~\cite{Gollapalli:2013, Campbell:2003,Yeniterzi:2014,jiang2016exploiting,wang2013expertrank,faisal2019expert,bok2019expert,Sziklai:2018}, 
experts are represented as nodes, and their relationships are represented by their edges or implicitly derived from a  graph. Different algorithms were used in the GM approach, such as Hyperlink-Induced Topic Search (HITS)  \cite{Campbell:2003, Yeniterzi:2014, jiang2016exploiting} and PageRank \cite{koumenides2014ranking}. 
% PageRank is an algorithm that was  designed to estimate the importance (i.e. authority) of a node in a network based on the link structure of the network. 
For expert finding, PageRank was adapted in the context of online community discussions on a user-user graph built based on votes from users whose questions were answered by whom~\cite{zhang2007expertise}. Also, a modified PageRank algorithm was developed and applied for finding experts in online knowledge communities~\cite{wang2013expertrank}.
HITS is also a graph-based link analysis algorithm originally designed for ranking the importance of web pages based on authority and hub scores. The work~\cite{Campbell:2003} built an expert-expert bipartite graph based on email communication patterns and attempted to find the ranking of experts using HITS. 
CO-HITS was introduced~\cite{Hongbo:2009} to incorporate a bipartite graph with the content information from both sides (e.g. experts and documents in our context) by adding personalised parameters to HITS, and CO-HITS showed higher performance than HITS~\cite{Hongbo:2009}. Using an author-document-topic (ADT) graph, the expert finding GM model~\cite{Gollapalli:2013} leveraged possible paths between a topic and an expert on the ADT graph. Recently, diverse expert finding approaches were proposed in a social network. For example, the authors \cite{faisal2019expert} proposed a method for finding experts who can answer questions in a social network for `community question answering' using users' votes and reputations. The approach \cite{bok2019expert} focused on finding experts who can answer users’ questions based on 
users' online social activities in a social network (e.g. Twitter). 
% The work~\cite{Sziklai:2018} focused on finding experts based on the references of the authors in academia.

Also, we observe that some models tend to mix different techniques among DLM, VSM, and/or GM  \cite{kundu2019formulation}. For example,
%\yb{Again this is not for expert finding}.  
AuthorRank \cite{deng2011enhanced} combined a generative probabilistic DLM and a PageRank-like GM based on community engagement of expert candidates. The DLM was used to identify the most relevant documents, while the GM was used to model the authors’ authorities based on the community co-authorship.
The work~\cite{liu2013integrating} combined a cluster-based language model and a VSM for finding experts in question and answer communities. The authors \cite{kundu2019formulation} proposed a complex model for community question answering  using a variation of the DLM~\cite{Balog:2009} and a HITS-based GM (the HITS algorithm on a competition based expertise network~\cite{Aslay:2013}), where the scores from these models were linearly combined to rank experts given a question. 
The work~\cite{Mahani:2018} used the Dempster-Shafer combination theory to combine the DLM~\cite{Balog:2009} and a graph algorithm that analyses a social interaction of experts. However, this work did not provide technical details on how such combination is done.

Differing from the above approaches, \EF 
%in comparison with the related works are as follows: \amir{I think the first feature requires a better description. It is a bit hard to follow.} {\EF} 
is a first attempt in devising an ensemble model that incorporates $n$VSM  into \hits on an \ecg. The proposed   $n$VSM takes advantage of the IDF weighting for $N$-grams~\cite{nidf:2017}. \hits is a novel variation of CO-HITS and runs on an \ecg (i.e. expert-document bipartite graph), compared to previous works~\citep{Campbell:2003,Yeniterzi:2014}  that applied HITS on an expert-expert graph. 

% , where the weights of experts are estimated given a topic, but the prior works used topic-independent HITS algorithms~\citep{Campbell:2003,Yeniterzi:2014} for expert finding. 
% Third, \hits, the other key component in \EF, works on an expert-document graph, while these works~\citep{Campbell:2003,Yeniterzi:2014} applied HITS on an expert-expert graph. 
%Finally, we will also show \hits's outperformance over topic-sensitive CO-HITS. Further, we will conduct a comprehensive evaluation and show \EF's outperformance in comparison with the TFIDF-based VSM, DLM~\cite{Balog:2009,Wang:2015,WISER:2019} and GM approaches~\cite{Gollapalli:2013,Daniel:2015} in our evaluation.

% Although some HITS algorithms were previously used for expert finding, \EF differs in that (1) \hits is a \textit{topic-sensitive} HITS like algorithm, where the weights of experts are estimated given a topic, but the prior works used topic-independent HITS algorithms~\citep{Campbell:2003,Yeniterzi:2014}; 
% (2) \hits works on an \ecg, while \citep{Campbell:2003,Yeniterzi:2014} applied HITS on an expert-expert graph; and (3) \hits is a variation of CO-HITS~\citep{Hongbo:2009}. 
% In CO-HITS, an authority score (i.e. expert weight) is computed as the \textit{sum} of the hub scores (document weights) that point to that authority (expert). Also, a hub score is the \textit{sum} of the authority scores that the hub (document) points to. These authority and hub scores are mutually updated one another repeatedly. However, \hits calculates an authority score by the \textit{average} of the hub scores that point to that authority. Also, a hub score is calculated by the \textit{average} of the authority scores that the hub points to. 
% % Also, \hits is topic-sensitive, meaning that the authority and hub scores are calculated for a given topic.
% In our evaluation, we show the outperformance of \hits over CO-HITS.

% Existing literature on expert finding also proposed frameworks in areas such as data sources and data extraction process \cite{Rodrigo:2019}. Identifying a benchmark dataset  is a key component for evaluating an expertise finding model. A few research work focus on web-based datasource \cite{pal2015discovering}. Three benchmark dataset were introduced in  \cite{bordea2013benchmarking} from data about 590 conference workshops in Computer Science for expert finding. These dataset can be used in term-extraction or expertise topic extraction. The author evaluated expert finding and expert profiling tasks using three popular approaches - language modelling, document count and topic-centring and found that the topic-centring approach outperforms the simple \textit{TF-IDF} method \cite{riahi2012finding} and achieved mean average precision of 0.0392, 0.0369 and 0.0879 for three datasets. A test collection named TU expert collection is proposed by \cite{berendsen2013assessment} where expert users self-selected their topics and a the level of expertise for relevant areas. Such test collection can be used in evaluation and improvement of new expert finding model. This benchmark dataset is a valuable resource to evaluate and validate the new concept such as ExpFinder proposed in this paper.



%  In state-of-the-art two applications for expertise retrieval are mostly focused  - expert finding and expert profiling. ``Finding'' looks for experts related to a list of topics whereas ``Profiling'' focuses on identifying right topics for a given expert \cite{Rodrigo:2019}. Our developed ExpFinder model focuses on expert finding approach with the aim to identify candidate experts and ranking them based on their expertise topics and relevancy of similar experts.






% The ranking of documents according to the relevancy of expert is an important component of any expert finding model. One of efficient approach for such purpose is the vector-space model \cite{lu2013insight}. It  uses TF-IDF (term frequency-inverse document frequency) for assigning a score to a topic/document pair, in order to rank the documents. This  method  is  based  on  the  bag-of-words model \cite{wang2013expertrank}. The purpose of the ranking is to retrieve the most relevant documents from a collection. Ranking can directly affects retrieval quality. 
% \yb{TFIDF is a term-weighting scheme. I think we wouldn't need this para.}

% Existing literature on expert retrieval model also proposed various frameworks in areas such as data sources, data extraction process, expertise ranking, finding and profiling applications \cite{Rodrigo:2019}. To provide the reader to understand our approach and contribution this section provides a review of different expert finding approaches, ranking model and data source in details. 


%\subsection{Expert Finding based on Language Models}

% Language models \cite{husain2019expert, doval2019comparing}, also known as document-based or text-based approach, utilises aggregated text segments from multiple documents relevant to the expert. In this approach expert finding problem is mapped to multiple document features such as levels of associations between experts, and document authority information (e.g. pagerank, indegree). Such models estimates the relationships between topic and expert as the probability of generating a particular topic by a given expert \cite{van2016unsupervised}. For instance, two models are proposed based on probabilistic language modelling in \cite{balog2006formal} for expert finding. This is the first generation of the model based on a language model. The first model creates a textual representation of expert according to the documents and the second model ranks documents according to the topic query. The expert is determined based on associated documents.  BMExpert \cite{Wang:2015} used a weighted language model using three factors, relevance of documents to the query topic, importance of documents, and associations between documents and experts. The model then estimate the probability of a candidate being expert on a given topic and used that for ranking. \yb{Can we add more latest works using language models}

% A major drawback of language model is the number of relationships between experts and topics are very limited and the method of combining them are mostly heuristic and not clearly justified \cite{Rodrigo:2019}. \yb{any papers comparing the performance of language model-based approaches vs some other approaches? That'll be great if we can have such papers pinpointing the limitation vs performance....}


%\subsection{Expert Finding using Graphs}

% In recent literature of expert retrieval system, network or graph-based models are also used to represent the main topics of expertise finding models \cite{amjad2018ranking}. In such approach, graphs are used where experts represented as nodes and their relationships are by edges \cite{Gollapalli:2013}. There are many algorithms that are commonly used in graph-based models, such as Hyperlink-Induced Topic Search (HITS)  \cite{Kleinberg:1999, jiang2016exploiting}, topic modelling \cite{potha2019improving} and PageRank \cite{koumenides2014ranking}. 

% The effectiveness of graph-based methods proposed in \cite{Gollapalli:2013} for ranking experts using a weighted, undirected, tripirate graphs representing the Authors, Documents and Topics (ADT) in the corpus. In ADT model, authors used content-based  similarity between nodes and scored with respect to each other based on the association strengths of paths connecting them. Authors used three evaluation measure (MAP, MRR, Prec) over 2 experimental datasaets and showed that graph-based models are capable of providing a unified framework for ranking experts in response to both name and topic based search.

% In recent literature conventional web page ranking algorithms such as HITS and Pagerank has been used for expert finding in online communities \cite{zhang2007expertise,wang2013expertrank} \yb{2007 and 2013 are not recent :) Can we add more recent works - 2017 - 2020?}. HITS algorithm produces two values for a web page - its authority and its hub value. The potential of using HITS and PageRank algorithm in expert retrieval is proposed in \cite{zhang2007expertise} where authors addresses the issue of expert finding in an online help seeking community – the Java forums. Users' expertise profiles were constructed through their social network authority scores and posts terms. \yb{1. Can we add how HITS and Pagerank (with recen references) is used (key ideas of using a graph structure, objectives and approaches) for expert finding in more detail?}

% For our ExpFinder experiments we selected to use HITS  as  its values can be computed during query time and work well on a smaller document base. Scores estimated by HITS are also highly correlate with degree of linked nodes, which intuitively correspond to the level of expertise of an expert \cite{wang2013expertrank}. 

% \yb{Can we explain more about HITS-based, PageRank-based appraoches? How do they induce the expert profiling or matching?}


%\subsection{Expert Finding based on Hybrid Schemes}



% \subsection{Topic Weighting Schemes in Expert Finding}
% \yb{Can add a paragraph discussing topic weighting schemes in language based models in expert finding}

% \yb{Can add a paragraph discussing topic weighting schemes in graph based models in expert finding}

% In ExpFinder we have used TF-IDF \cite{riahi2012finding} as weighting mechanism for assigning score in topic and document. Such approach has been successfully used in literature in expert finding application areas. Authors in \cite{balog2008non} used TF-IDF for identifying non-local aspects of document-expert associations for their expert finding model in enterprise settings. Authors in \cite{chuang2014combining} used TF-IDF to identify ranking of extended terms associated with a query topic for an given expert. The authors obtained has 3\% higher precision than based using such approach. Authors in \cite{alhabashneh2017fuzzy} created fuzzy relevance profiles using TF-IDF analysis in their expert fiding systems. They combined three profiles into a unified index reflecting the semantic weight of the query terms related to the task, user and document to select the most relevant documents and experts related to the query topic. 


% \subsection{Evaluation Data Sources}
% Identifying a benchmark dataset  is a key component for evaluating = an expertise finding model. A few research work focus on web-based datasource \cite{pal2015discovering}. Three benchmark dataset were introduced in  \cite{bordea2013benchmarking} from data about 590 conference workshops in Computer Science for expert finding. These dataset can be used in term-extraction or expertise topic extraction. The author evaluated expert finding and expert profiling tasks using three popular approaches - language modelling, document count and topic-centring and found that the topic-centring approach outperforms the simple \textit{TF-IDF} method \cite{riahi2012finding} and achieved mean average precision of 0.0392, 0.0369 and 0.0879 for three datasets. 

% A biomedical domain datasource  is used in BMExpert \cite{Wang:2015}. The benchmark dataset used for the evaluation has 14 different topics relevant to the MEDLINE publications of program committee members in ISMB between 2012 and 2014. Authors used average precision (AP) value for evaluation and BMExpert achieved highest average P@50 of 6.71 in compare to GoPubMed (3.86\%), Jane (3.14\%) and eTBLAST (2.14\%). Although the weighted language model as proposed in BMExpert achieved good performance in finding experts in compare to some state-of-the art. However, the proposed approach only rely on three properties of documents, i.e., recentness, impact factor and the specific domain.  Moreover, for the document-expert associations, the authors considered only the first and last authors instead of all authors. 

% A test collection named TU expert collection is proposed by \cite{berendsen2013assessment} where expert users self-selected their topics and a the level of expertise for relevant areas. Such test collection can be used in evaluation and improvement of new expert finding model. This benchmark dataset is a valuable resource to evaluate and validate the new concept such as ExpFinder proposed in this paper.





% Authors in \cite{Vitor:2016} proposed an expert retrieval system named Lattes Expertise Retrieval (LExR) which provides a comprehensive, large-scale benchmark for evaluating expertise retrieval approaches, in particular, academic expertise retrieval. LExR is based on two type of retrieval task. One is \textit{expert profiling} that identifies topics of expertise for a given expert, and the other one is \textit{expert finding} that identify experts for a given topic. The authors evaluated their approach on a large-scale dataset that contains information of experts from all knowledge areas working in research institutions all over Brazil along with graded judgements of topics of expertise. In total, 235 obtained topics associated with 1635 experts in their proposed benchmark dataset.  

% \subsection{ExpFinder vs Existing Approaches}
% \yb{Later on, we can add this section}
